The extension of Weyl-type relative perturbation bounds

We extend several relative perturbation bounds to Hermitian matrices that are possibly singular, and also develop a general class of relative bounds for Hermitian matrices. As a result, corresponding relative bounds for singular values of rank-deficient $m\times n$ matrices are also obtained using the Jordan-Wielandt matrices. We also present that the main relative bound derived would be invariant with respect to congruence transformation under certain conditions, and compare its sharpness with the Weyl's absolute perturbation bound.

==> contents.tex/Chapter_1.tex <==
\section{Weyl-type relative bounds for eigenvalues}
\subsection{The main Weyl-type relative bound}
The main relative perturbation bound of this section stems from Theorem 2.3 in [10] and a special case of Theorem 2.1 in [11] which states that if $A$ and $A+E$ are positive definite and $k=\|A^{-1/2}EA^{-1/2}\|$, we get $\lambda_i(A)-k|\lambda_i(A)|\leq \lambda_i(A+E)\leq \lambda_i(A)+k|\lambda_i(A)|$. [4, Theorem 2.1] extends this result to when $A$ is Hermitian non-singular by imposing the additional constraint that $k\leq 1$. A question that naturally arises is if the analogue holds if we relax the assumption and allow $A$ to not have full rank, and do a similar derivation but also deal with $A$ being potentially singular. 

The idea used to prove Theorem 2.1 in [4] is to first show that $-kP\leq E \leq  kP$ where $P$ is the polar factor of $A$ then apply the monotonicity theorem for Hermitian matrices [7, Corollary 4.3.12]. We are going to show that a slight generalisation of the result holds without assuming  that $A$ is non-singular, by following a similar approach but instead of $A^{-1}$ we consider the pseudo inverse $A^+$ which always exists. 
 \begin{theorem}
Let $A$ be Hermitian with rank $r\leq n$ and eigenvalues $\lambda_1\geq...\geq \lambda_r, \lambda_{r+1}=...=\lambda_n=0$. Let $E$ be Hermitian and the eigenvalues of $A+E$ be in decreasing order.   If $k=\|(A^{1/2})^{+} E(A^{1/2})^{+}\|\leq 1$, we have for any $i\in \{1,...,r\},$
\begin{equation}
\lambda_{n-r+i}(A+E)\leq \lambda_i+k|\lambda_i|
    \end{equation}
and \begin{equation}
    \lambda_i(A+E) \geq \lambda_i -k|\lambda_i|
\end{equation}
   
\begin{proof}
 Take the (thin) spectral decomposition $A=VDV^*=V_rD_rV_r^*$ and hence its polar factorisation $A=PS=SP$ where $P$ is positive semi-definite and $S$ is unitary. Denote $H_r=\mbox{sign}(D_r)$, then \begin{equation*}
     P=\left[\begin{array}{cc}
        V_r  &  V_r^\perp
         \end{array}\right] \left[\begin{array}{cc}
     |D_r| &  \\
      & \mathbf{0}
 \end{array}\right] \left[\begin{array}{cc}
      V_r^*  \\
      {V_r^{\perp}}^*
 \end{array}\right]
\end{equation*}
\begin{equation*}
S=\left[\begin{array}{cc}
    V_r &  V_r^\perp
\end{array}\right] \left[\begin{array}{cc}
     H_r &  \\
      & I 
 \end{array}\right] \left[\begin{array}{cc}
      V_r^*  \\
     {V_r^{\perp}}^*
 \end{array}\right]
 \end{equation*}
 Using the characterisation of pseudo inverse via SVD, \begin{equation*} \begin{array}{cc}
(A^{1/2})^+=V_rD_r^{-1/2}V_r^* &(P^{1/2})^+=V_r|D_r|^{-1/2}V_r^* \end{array}
\end{equation*} Following the approach in [4], since for all $1 \leq j \leq r, 
    \lambda_j^{1/2}=(\mbox{sign}(\lambda_j))^{1/2}|\lambda_j|^{1/2}$, we have
    $\frac{(sign(\lambda_j))^{1/2}}{\lambda_j^{1/2}}=|\lambda_j|^{-1/2} $ where $(\mbox{sign}(\lambda_j))^{1/2}$ are entries of $H_r^{1/2}$, $\lambda_j^{-1/2}$ are entries of $D_r^{-1/2}$ and $ |\lambda_j|^{-1/2}$ are entries of $|D_r|^{-1/2}$. As a result,  \begin{equation*}
|D_r|^{-1/2}=D_r^{-1/2}H_r^{1/2}=H_r^{1/2}D_r^{-1/2}\end{equation*}
Therefore, \begin{equation} \begin{aligned}
    (P^{1/2})^{+}
    &=(V_rD_r^{-1/2}V_r^*)(V_rH_r^{1/2}V_r^*)\\
    &=V_rD_r^{-1/2}V_r^*\left[\begin{array}{cc}
         V_r & V_r^\perp 
    \end{array}\right] \left[\begin{array}{cc}
     H_r^{1/2}&  \\
      & I 
 \end{array}\right]\left[\begin{array}{cc}
      V_r^*  \\
      {V_r^{\perp}}^*
 \end{array}\right]\\
    &=(A^{1/2})^{+}W=W(A^{1/2})^+
        \end{aligned}
    \end{equation} 
  where the last equality in (3) is obtained by re-doing the derivation but swapping $D_r^{-1/2}, H_r^{1/2}$ around since they commute as two diagonal matrices.


$W$ is unitarily diagonalisable with eigenvalues being roots of unity as shown in (3), so $W$ is unitary, which leads to
    \begin{equation}
        \begin{aligned}
        k&=\|(A^{1/2})^{+}E(A^{1/2})^{+}\|\\
        &= \|W(A^{1/2})^{+}E(A^{1/2})^{+}W\|\\
        &=\|(P^{1/2})^{+}E(P^{1/2})^{+}\|
        \end{aligned}
        \end{equation}
Since both $(P^{1/2})^+$ and $E$ are Hermitian, so is $(P^{1/2})^{+}E(P^{1/2})^{+}$. Following (4), we have $-kI_n \leq (P^{1/2})^{+}E(P^{1/2})^{+}\leq kI_n$.
 Multiplying all three sides both left and right by $P^{1/2}$ which is Hermitian preserves the order, and $(P^{1/2})^+P^{1/2}=P^{1/2}(P^{1/2})^+=V_rV_r^*$, we get $-kP\leq V_rV_r^*EV_rV_r^*\leq kP$. Adding $A$ to all sides gives \begin{equation*} 
 A-kP \leq A+V_rV_r^*EV_rV_r^* \leq A+kP
 \end{equation*} 
 Notice that $V_rV_r^*AV_rV_r^*=V_rV_r^*V_rD_rV_rV_r^*V_r^*=V_rD_rV_r^*=A$, so we have \begin{equation}
    A-kP\leq V_rV_r^*(A+E)V_rV_r^*\leq A+kP
\end{equation}
Applying the monotonicity theorem [7, Corollary 4.3.12] to (5) where all matrices are Hermitian, we get \begin{equation}
    \lambda_i (A-kP)\leq \lambda_i (V_rV_r^*(A+E)V_rV_r^*) \leq \lambda_i (A+kP)
\end{equation}


Our next aim is to find the correspondence between  $\lambda_i(V_rV_r^*(A+E)V_rV_r^*)$ and eigenvalues of $A+E$ to obtain (1) and (2) from (6). We can derive that for $i\in \{1,...,r\}$,  $\lambda_i(V_rV_r^*(A+E)V_rV_r^*)=\lambda_i(V_r^*(A+E)V_r)$ by applying the result that $\mbox{eig}(XY)=\mbox{eig}(YX)$ [7, Theorem 1.3.22] repeatedly: for $i\in \{1,...,r\}$, \begin{equation*} \begin{aligned}
    \lambda_i(\underbrace{V_rV_r^*}_X\underbrace{(A+E)V_rV_r^*}_Y)&=\lambda_i((A+E)(V_rV_r^*V_rV_r^*))\\
    &=\lambda_i((A+E)V_rV_r^*)\\
    &=\lambda_i(V_r^*(A+E)V_r)
\end{aligned}
\end{equation*}
Consider $V_r^*(A+E)V_r$ in relation to $A+E$: \begin{equation} \begin{aligned}
    V^*(A+E)V&= \left[\begin{array}{cc}
       V_r^*  \\
       {V_r^{\perp}}^*
    \end{array}\right](A+E) \left[\begin{array}{cc}
        V_r & V_r^\perp
        \end{array}\right] \\
    &=\left[\begin{array}{cc}
       V_r^*(A+E)V_r  & V_r^*(A+E)V_r^\perp \\
        {V_r^{\perp}}^*(A+E)V_r & {V_r^{\perp}}^*(A+E)V_r^\perp
    \end{array}\right]
\end{aligned}
\end{equation}
Hence, $V_r^*(A+E)V_r$ is the $r\times r$ principal sub-matrix of $V^*(A+E)V$, both of which are Hermitian. Using Theorem 4.3.28 in [7], we get for $i\in \{1,...,r\}$, \begin{equation}\lambda_{n-r+i}(V^*(A+E)V)\leq \lambda_i(V_r^*(A+E)V_r)\leq \lambda_i(V^*(A+E)V) \end{equation} But $V^*(A+E)V$ is unitarily similar to $A+E$ meaning their eigenvalues are identical, so (8) becomes $\lambda_{n-r+i}(A+E)\leq \lambda_i(V_r^*(A+E)V_r)\leq \lambda_i(A+E)$. Combining this with (6), we get for $i\in\{1,...,r\}$, \begin{equation} \begin{aligned}
     \lambda_{n-r+i}(A+E)&\leq \lambda_i(V_r^*(A+E)V_r)\\
     &= \lambda_i(V_rV_r^*(A+E)V_rV_r^*)\\
     &\leq \lambda_i(A+kP)
     \end{aligned} 
\end{equation}
and \begin{equation} \begin{aligned}
    \lambda_i(A+E)&\geq \lambda_i(V_r^*(A+E)V_r)\\
    &=\lambda_i(V_rV_r^*(A+E)V_rV_r^*)\\
    &\geq \lambda_i(A-kP)
\end{aligned}
    \end{equation}
 where $A \pm kP= V_r (D_r \pm k|D_r|) V_r^*$.  $k\leq 1$ is sufficient to ensure that $\lambda_j \leq \lambda_{j'}$ always implies that $\lambda_j \pm k|\lambda_j|\leq \lambda_{j'}\pm k|\lambda_{j'}| $, because the functions $f, g:\mathrm{R} \rightarrow \mathrm{R}$ defined by $f(x)=x + k|x|, g(x)=x-k|x|$ are increasing over $\mathrm{R} $ when $k\leq 1$. So for any $i$, \begin{equation}
 \lambda_i (A \pm kP)= \lambda_i \pm k|\lambda_i| \end{equation}
 Substituting (11) into (9) and (10) for $i\in \{1,...,r\}$, we get $\lambda_{n-r+i}(A+E)\leq \lambda_i +k|\lambda_i|$ and $ \lambda_i(A+E)\geq \lambda_i-k|\lambda_i|$ ,  which is (1) and (2) respectively. 
\end{proof}
\end{theorem}
\begin{remark} \textnormal{When $A$ is non-singular it has full rank. Substituting $r=n$ into (1) and (2) we get $\lambda_i-k|\lambda_i|\leq \lambda_i(A+E)\leq \lambda_i+k|\lambda_i| $ for any $i\in \{1,...,n\}$ so we recover Theorem 2.1 in [4]. Also as pointed out in [4], the condition $k\leq 1$ is necessary in order to have $\lambda_i (A \pm kP)= \lambda_i \pm k|\lambda_i|$ because when $k>1$, take $ |\lambda_j|\gg|\lambda_{j'}|$ while $\lambda_j<0$, $\lambda_{j'}>0$, then $\lambda_j+k|\lambda_j|>\lambda_{j'}+k|\lambda_{j'}|$ so (11) is not true in this case. Even when just $A$ is positive semi-definite so $\lambda_l\geq 0$ for all $l$, (11) does not hold in general for $k>1$, because the function $g(x)=x-k|x|$ is decreasing on $[0, \infty)$ when $k>1$. }
\end{remark}
However, following the argument in [4], we can drop the constraint that $k\leq 1$ whenever both $A, A+E$ are positive semi-definite and hence recover an analogue of Corollary 4.2 in [6] and Theorem 2.3 in [10]:
\begin{corollary}
Let $A$ be positive semi-definite with rank $r\leq n$ and eigenvalues $\lambda_1\geq...\geq \lambda_r>0=\lambda_{r+1}=...=\lambda_n$. Let $A+E$ also be  positive semi-definite with eigenvalues in decreasing order, $k=\|(A^{1/2})^+E(A^{1/2})^+\|$. Then for any $i\in \{1,...,r\}$, 
\begin{equation*} 
\begin{array}{cc}
\lambda_{n-r+i}(A+E)\leq \lambda_i+k\lambda_i, & \lambda_i(A+E) \geq \lambda_i -k\lambda_i\\
\end{array}
\end{equation*}
   \end{corollary}
    \begin{proof}
        We follow the same proof as in Theorem 2.1 until obtaining (9) and (10). 
 
 Recall $A \pm kP= V_r (D_r \pm k|D_r|) V_r^*$. Since $A$ is positive semi-definite, $\lambda_l\geq 0$ for all $l$. As a result, for any $k,  \lambda_j\leq \lambda_{j'}$ implies that $\lambda_j +k\lambda_j\leq \lambda_{j'}+k\lambda_{j'}$, which means $\lambda_i(A+kP)=\lambda_i+k\lambda_i$ for any $i$. Substituting in (9), we get for any $i\in \{1,...,r\}, \lambda_{n-r+i}(A+E)\leq \lambda_i(A+kP)=\lambda_i+k\lambda_i$.
 
On the other hand, for any $i\in \{1,...,r\}$, when $k>1,$ $\lambda_i-k\lambda_i\leq 0$, while $\lambda_i(A+E)\geq 0$ because $A+E$ is positive semi-definite, so $\lambda_i-k\lambda_i\leq \lambda_i(A+E).$ We have shown that this also holds when $k\leq 1$ in Theorem 2.1, so $\lambda_i(A+E)\geq \lambda_i-k\lambda_i$ for any values of $k$ as well.     \end{proof}

$\|(A^{1/2})^+E(A^{1/2})^+\|$ may be hard to compute as it involves $A^{1/2}$ and its pseudo inverse. We will give a practical method to compute it when $A$ is non-singular in Section 3.3. It is also not the only choice of $k$ to give a relative bound. In [4], [6] and [8], other choices of  $k$ besides $\|A^{-1/2}EA^{-1/2}\|$ are $\|A^{-1}E\|$ and $\|EA^{-1}\|$ which can also be used in giving a relative bound of the form (1) and (2) when $A$ has full rank. We will show that using a similar reasoning as in the proof of [4, Lemma 2.2], $\|A^+E\|$ or $\|EA^{+}\|$ can replace $\|(A^{1/2})^+E(A^{1/2})^+\|$ in Theorem 2.1. 
\begin{theorem}
Let $A$ be  Hermitian with rank $r\leq n$ and eigenvalues $\lambda_1\geq...\geq \lambda_r, \lambda_{r+1}=...=\lambda_n=0$. Let $E$ be Hermitian and the eigenvalues of $A+E$ be in decreasing order. If $k\in \{\|A^+E\|, \|EA^+\|\}\leq 1$, we have for any $i\in \{1,...,r\},$
\begin{equation*} 
\begin{array}{cc}
\lambda_{n-r+i}(A+E)\leq \lambda_i+k|\lambda_i|, & \lambda_i(A+E) \geq \lambda_i -k|\lambda_i|\\
\end{array}
    \end{equation*}
 \begin{proof}
        It suffices to show that $\|(A^{1/2})^+E(A^{1/2})^+\|\leq \|A^+E\|=\|EA^+\|$, then the result is a consequence of Theorem 2.1 with the new $k$. Since $A=V_rD_rV_r^*$ is Hermitian, $A^+=V_rD_r^{-1}V_r^*$ is Hermitian. Then \begin{equation}
            \|A^+E\|=\|(A^+E)^*\|=\|E^*(A^+)^*\|=\|EA^+\|
        \end{equation}
Take the polar decomposition $A=PS=SP$ where $P=V_r|D_r|V_r^*.$ Using (4), $\|(A^{1/2})^+E(A^{1/2})^+\|=\|(P^{1/2})^+E(P^{1/2})^+\|.$
As $(P^{1/2})^+=V_r|D_r|^{-1/2}V_r^*$ is Hermitian, $(P^{1/2})^+E(P^{1/2})^+$ is Hermitian. Therefore, 
\begin{equation}
\begin{aligned}
     \|(P^{1/2})^+E(P^{1/2})^+\|&=\max\limits_i|\lambda_i(\underbrace{(P^{1/2})^+}_{X}\underbrace{E(P^{1/2})^+}_{Y})|\\
     &=\max\limits_i|\lambda_i(E(P^{1/2})^+(P^{1/2})^+)|\\
     &=\max\limits_i|\lambda_i(EP^+)|\\
     &\leq \|EP^+\|=\|E(P^+S)\|=\|EA^+\|
     \end{aligned}
\end{equation}
where the second line uses the result $\mbox{eig}(XY)=\mbox{eig}(YX)$ [7, Theorem 1.3.22] and final line uses $A^+=V_rD_r^{-1}V_r^*=(V_r|D_r|^{-1}V_r^*)(V_r H_rV_r^*)=P^+S$ where $H_r=\mbox{sign}(D_r^{-1})$ and $S= V\left[\begin{array}{cc}
     H_r &  \\
      & I 
 \end{array}\right]V^*$ is unitary.
\end{proof}
\end{theorem}
 Motivated by the derivation of Theorem 2.2, the inequalities in (12) and (13) should hold in a more general context, as illustrated by the result below using the same idea as Lemma 2.2 in [4].
\begin{observation*}
    Let $A,C$ be two normal matrices with the same polar factor. If $B$ is normal, then $\|AB\|=\|BC\|$. If $B$ is Hermitian, then $\|A^{1/2}BC^{1/2}\|\leq \|AB\|=\|BC\|$ \end{observation*}
 \begin{proof}
     Let $A=PS=SP, C=PQ=QP, B=P_BU=UP_B$ be their polar decomposition where $P, P_B$ are positive semi-definite and $S,Q,U$ are unitary. We have \begin{equation*}
\|AB\|=\|SPP_BU\|=\|PP_B\|=\|P_B^*P^*\|=\|P_BP\|=\|UP_BPQ\|=\|BC\|
     \end{equation*}
Repeating the derivation in (3) but now for $P^{1/2}$, we get $P^{1/2}=A^{1/2}W_A=W_AA^{1/2}$ and $P^{1/2}=C^{1/2}W_B$. When $B$ is Hermitian, following (13): \begin{equation*} \begin{aligned}
   \|AB\|&=\|SPB\|=\|PB\|\geq\max\limits_i|\lambda_i(PB)|\\ 
   &= \max\limits_i|\lambda_i(\underbrace{P^{1/2}}_X\underbrace{P^{1/2}B}_Y)|=\max\limits_i|\lambda_i(P^{1/2}BP^{1/2})|\\
   &=\|P^{1/2}BP^{1/2}\|=\|W_AA^{1/2}BC^{1/2}W_B\|=\|A^{1/2}BC^{1/2}\|
\end{aligned}   
\end{equation*} In particular, taking $C=A$ leads to $\|A^{1/2}BA^{1/2}\|\leq \|AB\|=\|BA\|$ for any $A$ normal and $B$ Hermitian with agrees with [4, Lemma 2.2].\end{proof}  

 \subsection{A class of Weyl-type relative bounds}
Having seen relative bounds of the form (1) and (2) where the choices of $k$ can be $\|(A^{1/2})^+E(A^{1/2})^+\|$, $\|A^+E\|$ and $\|EA^+\|$, a follow-up question is that whether they belong to a larger class of relative perturbation bounds. The motivating result of this mainly comes from [6, Corollary 2.4] giving a general form of Bauer-Fike type relative bounds, which we will state below:
\begin{theorem}[Eisenstat and Ipsen, 1995]
    Let $A$ be a non-singular diagonalisable matrix. If $A=A_1A_2=A_2A_1$ and $\kappa (X)$ is the conditional number of eigenvector matrix of $A$, then for any given eigenvalue $\lambda (A+E)$, \begin{equation*}
        \min\limits_i\frac{|\lambda_i(A)-\lambda(A+E)|}{|\lambda_i(A)|}\leq \kappa (X)\|A_1^{-1}EA_2^{-1}\|
    \end{equation*}
    \end{theorem}
    It was proven in [6] by applying the Bauer-Fike theorem in [1] to $A_2AA_2^{-1}$ and $A_2EA_2^{-1}$.  We would like to establish a similar result for $A, E$ being Hermitian not only with an one-to-one pairing between $\lambda_i(A+E)$ and $\lambda_i(A)$ for the same index $i$, but also take into account that  $A_1, A_2$ can be singular, in order to find a form of relative bounds extending Theorem 2.1 and 2.2. In the following theorem we are going to present a class of relative bounds and it will be used later to give an analogue of Theorem 2.3 in the case that $A, E$ are both Hermitian. 



 \begin{theorem}
Let $A$ be Hermitian of rank $r\leq n$ and eigenvalues $\lambda_1\geq...\geq \lambda_r, \lambda_{r+1}=...=\lambda_n=0$, and polar factor $P$. Let $E$ be Hermitian, $P_1$ be the left polar factor of $A_1$, $P_2$ be the right polar factor of $A_2$. If $P=P_1P_2=P_2P_1$ and $k=\|A_1^+EA_2^+\|\leq 1$, then for any $i\in \{1,...,r\},$
\begin{equation}
\begin{array}{cc}
\lambda_{n-r+i}(A+E)\leq \lambda_i+k|\lambda_i|, & \lambda_i(A+E) \geq \lambda_i -k|\lambda_i|
\end{array}\end{equation}        
where the eigenvalues of $A+E$ are in decreasing order.
\end{theorem}
\begin{proof}
  Let $A=VDV^*=V_rD_rV_r^*$ be its unitary diagonalisation with its eigenvalues arranged in the specified ordering above, then $P=V|D|V^*=V_r|D_r|V_r^*$ as its unitary diagonalisation.  Since $PP_1=P_1P_2P_1=P_1P,$ $ PP_2=P_2P_1P_2=P_2P$
 and $P_1P_2=P_2P_1$, we have $P, P_1, P_2$ forming a commuting family. Since they are all Hermitian, by Theorem 2.5.5 in [7], $P_1$ ,$P_2$ are also diagonalisable through $V$. 
Let \begin{equation*}
    P_1=V\Lambda V^*=\left[\begin{array}{cc}
        V_r  &  V_r^\perp
         \end{array}\right] \left[\begin{array}{cc}
     \Lambda_r &  \\
      & \Lambda_{n-r}
 \end{array}\right] \left[\begin{array}{cc}
      V_r^*  \\
      {V_r^{\perp}}^*
 \end{array}\right]\end{equation*}
 \begin{equation*}
      P_2=V\Sigma V^*=\left[\begin{array}{cc}
        V_r  &  V_r^\perp
         \end{array}\right] \left[\begin{array}{cc}
     \Sigma_r &  \\
      & \Sigma_{n-r}
 \end{array}\right] \left[\begin{array}{cc}
      V_r^*  \\
     {V_r^{\perp}}^*
 \end{array}\right] \end{equation*}
where $\Lambda, \Sigma $ are diagonal with entries being the eigenvalues of $P_1, P_2$ without specific ordering. Since $P=P_1P_2$, we have $V|D|V^*=V\Lambda\Sigma V^*$. Multiplying its both sides by $V^*$ on the left and $V$ on the right, we have \begin{equation}
     \left[\begin{array}{cc}
     |D_r| &  \\
      & \mathbf{0}
 \end{array}\right] = \left[\begin{array}{cc}
     \Lambda_r\Sigma_r &  \\
      & \Lambda_{n-r}\Sigma_{n-r}
 \end{array}\right] 
 \end{equation}
As a result, both $\Lambda_r$ and $\Sigma_r$ are invertible because all diagonal entries of $|D_r|$ are non-zero. Let  $F=V \left[\begin{array}{cc}
    \Lambda_r^{-1} &  \\
      & \Lambda_{n-r}^+
 \end{array}\right]V^*$. Then \begin{equation*}
    P_1FP_1=V\left[\begin{array}{cc}
    \Lambda_r\Lambda_r^{-1}\Lambda_r&  \\
      & \Lambda_{n-r}\Lambda_{n-r}^+\Lambda_{n-r}
 \end{array}\right]V^* = V \left[\begin{array}{cc}
    \Lambda_r &  \\
      & \Lambda_{n-r}
 \end{array}\right]V^*   =P_1 \end{equation*}
 \begin{equation*}
     FP_1F=V\left[\begin{array}{cc}
    \Lambda_r^{-1}\Lambda_r\Lambda_r^{-1}&  \\
      & \Lambda_{n-r}^+\Lambda_{n-r}\Lambda_{n-r}^+
 \end{array}\right]V^*= V\left[\begin{array}{cc}
    \Lambda_r^{-1}&  \\
      & \Lambda_{n-r}^+
 \end{array}\right]V^*=F \end{equation*}
\begin{equation*} \begin{array}{cc}
 FP_1=V \left[\begin{array}{cc}
     I_r  &  \\
     & \Lambda_{n-r}^+\Lambda_{n-r}
  \end{array}\right]V^*,   & P_1F=V\left[\begin{array}{cc}
      I_r &  \\
       & \Lambda_{n-r}\Lambda_{n-r}^+
  \end{array}\right]V^*  
\end{array}
 \end{equation*}
 where $FP_1$ and $P_1F$ are Hermitian because $\Lambda_{n-r}^+\Lambda_{n-r}$ and $\Lambda_{n-r}\Lambda_{n-r}^+$ are Hermitian. Hence, $P_1^+=F=V\left[\begin{array}{cc}
     \Lambda_r^{-1}  &  \\
     & \Lambda_{n-r}^+\
  \end{array}\right]V^*$. Similarly, $P_2^+=V\left[\begin{array}{cc}
     \Sigma_r^{-1}  &  \\
     & \Sigma_{n-r}^+
  \end{array}\right]V^*$. In addition, we can express $A_1^+, A_2^+$ in terms of $P_1^+, P_2^+$:  Since $A_1=P_1S_1$ with $S_1$ being unitary, and $A_2=S_2P_2$ with $S_2$ being unitary, we have $A_1^+=S_1^*P_1^+$ and $A_2^+=P_2^+S_2^*$. 

Therefore, \begin{equation*}
k=\|A_1^+EA_2^+\|=\|S_1^*P_1^+EP_2^+S_2^*\|=\|P_1^+EP_2^+\|
 \end{equation*}
Our next aim is to show that \begin{equation}
     A-kP\leq A+V_rV_r^*EV_rV_r^*\leq A+kP
      \end{equation}     
      because if this holds,  using the same reasoning starting from (5) in Theorem 2.1, we can obtain (14). Let $P_1^r=V_r\Lambda_rV_r^*$ and $P_2^r=V_r\Sigma_r V_r^*$, then
      \begin{equation*}
\begin{aligned}
    P_1^rP_1^+&=V\left[\begin{array}{cc}
         \Lambda_r &  \\
          & \mathbf{0}
     \end{array}\right]V^*V\left[\begin{array}{cc}
        \Lambda_r^{-1} &  \\
         & \Lambda_{n-r}^+
    \end{array}\right]V^* \\
    &=\left[\begin{array}{cc}
        V_r & V_r^\perp
    \end{array}\right]\left[\begin{array}{cc}
       I_r  &  \\
         & \mathbf{0}
    \end{array}\right]\left[\begin{array}{cc}
       V_r^*    \\
         {V_r^{\perp}}^*
    \end{array}\right]=V_rV_r^*
    \end{aligned}
 \end{equation*}
  Similarly, $P_2^+P_2^r=V\left[\begin{array}{cc}
     \Sigma_r^{-1}  &  \\
       & \Sigma_{n-r}^+
  \end{array}\right]\left[\begin{array}{cc}
     \Sigma_r  &  \\
       & \mathbf{0}
  \end{array}\right]V^*=V_rV_r^*$. Therefore, we have \begin{equation}
P_1^rP_1^+EP_2^+P_2^r=V_rV_r^*EV_rV_r^*
  \end{equation} When $k=\|P_1^+EP_2^+\|=0$, $P_1^+EP_2^+=\mathbf{0}$ and  $V_rV_r^*EV_rV_r^*=\mathbf{0}$ by (17), so (16) always holds. We can assume $k>0$ from now on.  
  To show that $ P_1^rP_1^+EP_2^+P_2^r\leq kP$, both of which are Hermitian, is equivalent to showing all eigenvalues of $kP-P_1^rP_1^+EP_2^+P_2^r$ are positive.  Using [7, Theorem 1.3.22], for non-zero eigenvalues, \begin{equation*}
  \begin{aligned}
      \mbox{eig}(kP-P_1^rP_1^+EP_2^+P_2^r)&=\mbox{eig}(V_rk|D_r|V_r^*-V_rV_r^*EV_rV_r^*)\\
      &=\mbox{eig}(V_r(k|D_r|-V_r^*EV_r)V_r^*)\\
      &=\mbox{eig}(k|D_r|-V_r^*EV_r)
  \end{aligned}
  \end{equation*}
  Hence, the eigenvalues of $kP-P_1^rP_1^+EP_2^+P_2^r$ are all the $r$ eigenvalues of $k|D_r|-V_r^*EV_r$ together with $n-r$ copies of zeros by [7, Theorem 1.3.22], so it suffices to show that all eigenvalues of $k|D_r|-V_r^*EV_r$ are non-negative. Let $\Tilde{A}=k|D_r|$ and  $\Tilde{E}=-V_r^*EV_r$. By applying (2) in Theorem 2.1, we get for all $i\in\{1,...,r\}$, \begin{equation}
     \lambda_i(\Tilde{A}+\Tilde{E} )\geq \lambda_i(\Tilde{A})-\|\Tilde{A}^{-1/2}\Tilde{E}\Tilde{A}^{-1/2}\|\lambda_i(\Tilde{A})
  \end{equation}
where  $\Tilde{E}=-V_r^*(V_rV_r^*EV_rV_r^*)V_r=-V_r^*P_1^rP_1^+EP_2^+P_2^rV_r$ by (17) is Hermitian and $\Tilde{A}^{-1/2}=k^{-1/2}|D_r|^{-1/2}$ where $|D_r|^{-1/2}$ is Hermitian.  Then using $\mbox{eig}(XY)=\mbox{eig}(YX)$, \begin{equation}
  \begin{aligned}
      \|\Tilde{A}^{-1/2}\Tilde{E}\Tilde{A}^{-1/2}\| 
      &=k^{-1}\||D_r|^{-\frac{1}{2}}V_r^*P_1^rP_1^+EP_2^+P_2^rV_r|D_r|^{-\frac{1}{2}}\|\\
      &=k^{-1}\max\limits_j|\lambda_j(\underbrace{|D_r|^{-\frac{1}{2}}V_r^*P_1^r}_{X}\underbrace{P_1^+EP_2^+P_2^rV_r|D_r|^{-\frac{1}{2}}}_{Y})|  \\ 
&=k^{-1}\max\limits_j|\lambda_j(P_1^+EP_2^+P_2^rV_r|D_r|^{-1}V_r^*P_1^r)|\\
&=k^{-1}\max\limits_j|\lambda_j(P_1^+EP_2^+P_2^rP^+P_1^r)|\\
\end{aligned}
    \end{equation}

 Recall (15), $|D_r|^{-1}=(\Lambda_r \Sigma_r)^{-1}=\Sigma_r^{-1}\Lambda_r^{-1}$,then 
  \begin{equation}
\begin{aligned}P_2^rP^+P_1^r&=V_r\Sigma_r V_r^*V_r|D_r|^{-1}V_r^*V_r\Lambda_r V_r^*\\
&=V_r\Sigma_r(\Sigma_r^{-1}\Lambda_r^{-1})\Lambda_rV_r^*\\
          &=V_rV_r^*
          \end{aligned}
      \end{equation}  
Hence, substituting (20) into (19), we have 
\begin{equation}
\begin{aligned}
\|\Tilde{A}^{-1/2}\Tilde{E}\Tilde{A}^{-1/2}\|&=k^{-1}\max\limits_j|\lambda_j(P_1^+EP_2^+V_rV_r^*)|\\
&\leq k^{-1}\|P_1^+EP_2^+V_rV_r^*\|\\&\leq k^{-1}\|P_1^+EP_2^+\|\|V_rV_r^*\|=k^{-1}k=1
\end{aligned}
\end{equation}
Combining (21) with (18) we have $  \lambda_i(\Tilde{A}+\Tilde{E} )\geq \lambda_i(\Tilde{A})-1\cdot\lambda_i(\Tilde{A})=0$ for any $i$. Therefore,  all $r$ eigenvalues of $k|D_r|-V_r^*EV_r$ are non-negative which shows that $kP-P_1^rP_1^+EP_2^+P_2^r$ is positive semi-definite, so $V_rV_r^*EV_rV_r^*=P_1^rP_1^+EP_2^+P_2^r \leq kP$. 

Similarly, $P_1^rP_1^+EP_2^+P_2^r \geq -kP$ is obtained by showing all eigenvalues of $kP+P_1^rP_1^+EP_2^+P_2^r $ are non-negative. This is again implied by $\lambda_i(k|D_r|+V_r^*EV_r)\geq 0$ for all $i\in \{1,...,r\}$, which can be obtained by repeating the derivation from (18) to (21) for $\Tilde{A}=k|D_r|$ and $\Tilde{E}=V_r^*EV_r.$ \footnote{The change in sign of $\Tilde{E}$ does not affect the related 2-norm or absolute value.} Hence, we have $ -kP\leq V_rV_r^*EV_rV_r^*\leq kP$, so (16) holds. If we now repeat the argument starting from (5) till the end in Theorem 2.1, we will obtain (14) for any $i\in\{1,..,r\}$, since $k\leq 1$.
\end{proof}
By swapping $A_1$ with $A_2$, we also get (14) for $i\in \{1,...,r\}$ with $k=\|A_2^+EA_1^+\|$, given that $P=P_1P_2=P_2P_1$ where $P_1$ is the right polar factor of $A_1$, $P_2$ is the left polar factor of $A_2$, following the same proof as Theorem 2.4. We can now give a class of relative bounds for Hermitian matrices that resembles Theorem 2.3 more:

\begin{corollary}
    Let $A$ be Hermitian with rank $r\leq n$ and eigenvalues $\lambda_1\geq...\geq \lambda_r, \lambda_{r+1}=...=\lambda_n=0$. If $A_1, A_2$ are normal matrices such that $A=A_1A_2=A_2A_1$,  $E$ is Hermitian and $k=\|A_1^+EA_2^+\|\leq 1$, then for any $i\in \{1,...,r\},$
\begin{equation*}
\begin{array}{cc}
\lambda_{n-r+i}(A+E)\leq \lambda_i+k|\lambda_i|, & \lambda_i(A+E) \geq \lambda_i -k|\lambda_i|
\end{array}\end{equation*}   
where the eigenvalues of $A+E $ are in decreasing order. 
\end{corollary}
\begin{proof}Since $AA_1=A_1A_2A_1=A_1A$ and $AA_2=A_2A_1A_2=A_2A$, $A, A_1$ and $ A_2$ form a commuting family of normal matrices. By [7, Theorem 2.5.5], there exists a unitary $V$ such that $A=VDV^*$ with eigenvalues arranged in the order specified above, and $A_1$ and $A_2$ can also be diagonalised through $V$. Let $A_1=V\Lambda V^*$ and $A_2=V\Sigma V^*$ where $\Lambda, \Sigma$ are diagonal which commute. Then $A=A_1A_2=V\Lambda\Sigma V^*$, so $D=\Lambda \Sigma$. The polar factors of $A_1, A_2$ are $P_1=V|\Lambda|V^*$ and $P_2=V|\Sigma|V^*$ respectively, while the polar factor of $A$ is $P=V|D|V^*=V|\Lambda||\Sigma|V^*$. Therefore we have $P=P_1P_2=P_2P_1$.  By Theorem 2.4, we get (14) for any $i\in \{1,...,r\}$, as $k\leq 1 $.\end{proof}
    
    In particular,  if we take $A_1=A^{1/2}=A_2$, since $A=VDV^*$ is Hermitian, $A^{1/2}=VD^{1/2}V^*$, so $A_1, A_2$ are normal with $A=A_1A_2=A_2A_1$. By Corollary 2.4.1, we get (14) with $k=\|(A^{1/2})^+E(A^{1/2})^+\|$, so we recover Theorem 2.1. Similarly, we can take $A_1=A$ and $A_2=I$, or $A_1=I$ and $A_2=A$. In both cases $A=A_1A_2=A_2A_1$ and they are all Hermitian. By Corollary 2.4.1 we obtain (14) with $k=\|A^+E\|$ and $k=\|EA^+\|$ respectively, recovering Theorem 2.2. 

In Corollary 2.4.1, we require both $A_1, A_2$ to be normal  to obtain (14) for $i\in \{1,...,r\}$, which is not needed in Theorem 2.3 as long as $A$ is non-singular.  We will show that the same conclusion can be reached without the assumption that $A_1, A_2$ are both normal, giving a special version of Theorem 2.3 when $A, E$ are Hermitian.

\begin{theorem}
    Let $A$ be Hermitian with rank $r\leq n$ and eigenvalues $\lambda_1\geq...\geq \lambda_r, \lambda_{r+1}=...=\lambda_n=0$, and let $E$ be Hermitian. If $A_1, A_2$ are matrices such that  $A=A_1A_2=A_2A_1$, and $k=\|A_1^+EA_2^+\|\leq1 $, then for any $i\in \{1,...,r\}$,\begin{equation*}
\begin{array}{cc}
\lambda_{n-r+i}(A+E)\leq \lambda_i+k|\lambda_i|, & \lambda_i(A+E) \geq \lambda_i -k|\lambda_i|
\end{array}\end{equation*}
 where the eigenvalues of $A+E$  are in decreasing order.\end{theorem}
 \begin{proof}
We consider $A_1A_1^*$ and $A_2^*A_2$. Since $A$ is Hermitian, \begin{equation*}
\begin{aligned}
    A_1A_2=A_2A_1=A=A^*&=(A_1A_2)^*=A_2^*A_1^*\\
    &=(A_2A_1)^*=A_1^*A_2^*
\end{aligned}
\end{equation*}
As a result, \begin{equation*}
    AA_1A_1^*=A_1A_2A_1A_1^*=A_1A_1^*A_2^*A_1^*=A_1A_1^*A
\end{equation*}
\begin{equation*}
    AA_2^*A_2=A_2^*A_1^*A_2^*A_2=A_2^*A_2A_1A_2=A_2^*A_2A
\end{equation*}
\begin{equation*}
    A_1A_1^*A_2^*A_2=A_1A_2A_1A_2=A_2^*A_1^*A_2^*A_1^*=A_2^*A_2A_1A_1^*
\end{equation*}
Hence, $A, A_1A_1^*$ and $A_2^*A_2$ form a commuting family of Hermitian matrices. By Theorem 2.5.5 in [7], there exists a unitary matrix $V$ which diagonalises $A$ with  $A=VDV^*$ where the eigenvalues are in the order specified above, and also $A_1A_1^*=V\Lambda_1V^*$ and $A_2^*A_2=V\Lambda_2V^*$ where $\Lambda_1, \Lambda_2$ are diagonal, so $A_1A_1^*A_2^*A_2=V\Lambda_1V^*V\Lambda_2V^*=V\Lambda_1\Lambda_2V^*=V\Lambda_2\Lambda_1V^*$. Since $A_1A_1^*, A_2^*A_2$ are positive semi-definite, there exist diagonal matrices $\Sigma_1, \Sigma_2$ with non-negative entries such that $\Lambda_1=\Sigma_1^2, \Lambda_2=\Sigma_2^2$. $A^2=VDV^*VDV^*=VD^2V^*$, and also \begin{equation*}
  A^2=(A_1A_2)(A_1A_2)=A_1(A_2A_1)A_2=A_1A_1^*A_2^*A_2=V\Sigma_1^2\Sigma_2^2V^*=V\Sigma_2^2\Sigma_1^2V^*
\end{equation*}
Hence, we have $D^2=\Sigma_1^2\Sigma_2^2=\Sigma_2^2\Sigma_1^2$, where $D$ has all real entries since $A$ is Hermitian, while $\Sigma_1, \Sigma_2$ have non-negative entries. Therefore, $|D|=\Sigma_1\Sigma_2=\Sigma_2\Sigma_1$, so the polar factor of $A$ is $P=V|D|V^*=V\Sigma_1\Sigma_2V^*=V\Sigma_2\Sigma_1V^*$. 

On the other hand, by Theorem 7.3.1 in [7], the left polar factor of $A_1=P_1S_1$ is $P_1=(A_1A_1^*)^{1/2}=(V\Sigma_1^2V^*)^{1/2}=V\Sigma_1V^*$, and the right polar factor of $A_2=S_2P_2$ is $P_2=(A_2^*A_2)^{1/2}=(V\Sigma_2^2V^*)^{1/2}=V\Sigma_2V^*.$ Therefore, we see $P=P_1P_2=P_2P_1$, so the conditions in Theorem 2.4 are satisfied. Since $k\leq 1$, we obtain (14) for $i\in \{1,...,r\}$ by applying Theorem 2.4. \end{proof}
\newpage
\begin{remark}
    \textnormal{When $A$ and $A+E$ are both positive semi-definite, the condition $k\leq 1$ can be dropped in Theorem 2.4, 2.5 and Corollary 2.4.1 because of the same reasoning as in Corollary 2.1.1 apart from the different definition of $k$ which does not play a role in the proof for it, resulting in an extension  of Corollary 2.1.1.} 
    
   \textnormal{Theorem 2.5 is easier to visualise than Theorem 2.4, and it gives a generalisation of Corollary 2.4.1. In particular, it incorporates all the previous choices of $k$ in Theorem 2.1 and Theorem 2.2, as explained in the proof of Corollary 2.4.1. }
\end{remark}
Finally, we note that when $A$ is not Hermitian in general, $A=A_1A_2=A_2A_1$ can still imply the same relation between their polar factors as in the proof of Theorem 2.5, provided that either of $A_1, A_2$ is normal. This could be useful in other context.
\begin{observation*}
Let $A_1, A_2$ be such that $A_1A_2=A_2A_1=A$ where $A=PS=SP'$ as its left and right polar decomposition. Let  $A_1=P_1S_1$ be its left polar decomposition and $A_2=S_2P_2$ be its right polar decomposition. Then if   $A_1$ is normal, we have $P'=P_1P_2=P_2P_1$, and if $A_2$ is normal, we have $P=P_1P_2=P_2P_1$
\end{observation*}
\begin{proof}First suppose $A_1$ is normal. By Fuglede-Putnam Theorem [7, Theorem 2.5.16],   $A_1A_2=A_2A_1$ implies that $A_1^*A_2=A_2A_1^*$, so $A_2^*A_1=(A_1^*A_2)^*=(A_2A_1^*)^*=A_1A_2^*$. As a result, $A_1A_2^*A_2=A_2^*A_1A_2=A_2^*A_2A_1$. Since $A_2^*A_2$ commutes with $A_1$, using [7, Theorem 2.5.5], there exists some unitary matrix $V$ such that $A_2^*A_2=VDV^*$ as its diagonalisation with eigenvalues arranged in decreasing order, and $A_1$ can also be diagonalised by $V$ as $A_1=V\Lambda V^*$, so its polar factor is $P=(A_1^*A_1)^{1/2}=V|\Lambda|V^*$.  Let $A_2=U\Sigma V^*$ be its SVD where $\Sigma\geq \mathbf{0}$ and $U$ is unitary. Then its right polar factor is $P_2=V\Sigma V^*$. Also, $A=A_2A_1=(U\Sigma V^*)(V\Lambda V^*)=U\Sigma \Lambda V^*$. By [7, Theorem 7.3.1],\begin{equation*}
    \begin{aligned}
        P'=(A^*A)^{1/2}&=(V\Lambda^*\Sigma U^*U\Sigma \Lambda V^*)^{1/2}\\
        &=(V|\Lambda|^2\Sigma^2V^*)^{1/2}\\
        &=V|\Lambda|\Sigma V^*=V\Sigma |\Lambda|V^*\\
        &=P_1P_2=P_2P_1
        \end{aligned}
    \end{equation*}

Similarly, let $A_2$ be normal. Using [7, Theorem 2.5.16], $A_2A_1=A_1A_2$ implies that $A_2A_1^*=(A_2^*A_1)^*=(A_1A_2^*)^*=A_1^*A_2$, so $A_2A_1A_1^*=A_1A_2A_1^*=A_1A_1^*A_2$. As before, there exists $W$ which is unitary that $A_1A_1^*=W\hat{D}W^*$ with its eigenvalues in decreasing order and $A_2=W\hat{\Lambda}W^*$. Let $A_1=W\hat{\Sigma}Q^*$ be its SVD where $\hat{\Sigma}\geq \mathbf{0}$, $Q$ is unitary. Then $P_1=W\hat{\Sigma}W^*$ and $P_2=W|\hat{\Lambda}|W^*$. Since $A=A_2A_1=W\hat{\Lambda}W^*W\hat{\Sigma}Q^*=W\hat{\Lambda} \hat{\Sigma}Q^*$, by [7, Theorem 7.3.1], \begin{equation*}
\begin{aligned}
    P=(AA^*)^{1/2}&=(W\hat{\Lambda}\hat{\Sigma}Q^*Q\hat{\Sigma}\hat{\Lambda}^*W^*)^{1/2}\\
    &=(W\hat{\Sigma}^2|\hat{\Lambda}|^2W^*)^{1/2}\\
    &=W\hat{\Sigma}|\hat{\Lambda}|W^*=W |\hat{\Lambda}| \hat{\Sigma} W^*\\
    &=P_1P_2=P_2P_1
    \end{aligned}
\end{equation*}\end{proof}






    
    
    
    
   



    

==> contents.tex/Chapter_2.tex <==
\section{Property and sharpness of the main result}
\subsection{Relation to congruence transformation}
As suggested by Theorem 2.5, there are various valid choices of $k$ for the relative bounds  $\lambda_{n-r+i}(A+E)\leq \lambda_i+k|\lambda_i|$,  $ \lambda_i(A+E) \geq \lambda_i -k|\lambda_i|$ where $A, E$ are Hermitian.  Among them, $k=\|(A^{1/2})^+E(A^{1/2})^+\|$, which is essentially Theorem 2.1, is perhaps more interesting as  it involves the same matrix $(A^{1/2})^+$ placing on both side of $E$. As shown by  [8, Corollary 2.2] and [10, Theorem 2.4], this choice of $k$ exhibits the property of being invariant  when $A, E$ both being positive definite are congruence transformed by the same invertible matrix $D$. In [6, Corollary 3.4], this is generalised to the case that $A$ is non-singular while its polar factor and $E$ are both congruence transformed by $D$. We will show that $A$ being potentially singular can also be taken into account by imposing one extra constraint on $D$, which vanishes when $A$ has full rank so the original theorems are recovered, and we will see that this constraint is both sufficient and necessary for the reverse order law to hold for the pseudo inverse of interest, which can also be obtained by [2, Theorem 3.1] and [9, Corollary 3.11]. 
\begin{theorem}
  Let $A$ be normal with rank $r\leq n$, an eigenvector matrix $V$ and polar factor $P$. If $\tilde{A}$ is normal with polar factor $\tilde{P}=DPD^*$, and $\tilde{E}=DED^*$ where $D$ is invertible such that $D^*D$ commute with $V_rV_r^*$, then \begin{equation}k=\|(A^{1/2})^+E(A^{1/2})^+\|=\|(\tilde{A}^{1/2})^+ \tilde{E}(\tilde{A}^{1/2})^+\|
       \end{equation}
    \end{theorem} 
    \begin{proof}
    We follow the same idea of proof as Corollary 3.4 in [6] but consider pseudo inverses instead.  Since $\Tilde{P}^{1/2}, P^{1/2}$ are Hermitian, $\Tilde{P}=\Tilde{P}^{1/2}\Tilde{P}^{1/2}=\Tilde{P}^{1/2}(\Tilde{P}^{1/2})^*$, and \begin{equation}
\Tilde{P}=DPD^*=DP^{1/2}P^{1/2}D^*=DP^{1/2}(P^{1/2})^*D^*=DP^{1/2}(DP^{1/2})^*
        \end{equation}
        Let $X=\Tilde{P}^{1/2}, Y=DP^{1/2}$. We see $XX^*=YY^*$ so they have the same spectral decomposition. Let $XX^*=YY^*=U\Lambda U^*$ with eigenvalues in decreasing order.  Then the SVD of $X$ is $X=U\Sigma Q_1^*$ where $\Sigma\geq \mathbf{0}$ and $Q_1$ is unitary. Similarly, the SVD of $Y$ is $Y=U\Sigma Q_2^*$ where $Q_2$ is unitary. Hence, $X=U\Sigma Q_2^*Q_2Q_1^*=YW$ where $W=Q_2Q_1^*$ is unitary, which means $\Tilde{P}^{1/2}=(DP^{1/2})W$. Taking pseudo inverse both side, since $W$ is unitary, $(\Tilde{P}^{1/2})^+=((DP^{1/2})W)^+=W^*(DP^{1/2})^+$. 

Consider $(DP^{1/2})^+$. It turns out that the condition of $D^*D$ commuting with $V_rV_r^*$ ensures that we have $(DP^{1/2})^+=(P^{1/2})^+D^{-1}$. If we first take $A=V\hat{\Lambda}V^*$ as its spectral decomposition, then $P=V|\hat{\Lambda}|V^*=V_r|\hat{\Lambda}_r|V_r^*$ and $P^+=V_r|\hat{\Lambda}_r|^{-1}V_r^*$ so we have $P^{1/2}(P^{1/2})^+=V_r|\hat{\Lambda}_r|^{1/2}V_r^*V_r|\hat{\Lambda}_r|^{-1/2}V_r^*=V_rV_r^*$. As a result, 
 \begin{equation}
 \begin{aligned}
    (DP^{1/2})(P^{1/2})^+D^{-1}=DV_rV_r^*D^{-1}
    \end{aligned}
    \end{equation}Since $D^*DV_rV_r^*=V_rV_r^*D^*D$ by the condition given, multiplying its both sides by $D^{-*}$ on the left and $D^{-1}$ on the right, we get \begin{equation*} 
\begin{aligned}
    DV_rV_r^*D^{-1}&=D^{-*}V_rV_r^*D^*\\
    &=(DV_rV_r^*D^{-1})^*
     \end{aligned}
\end{equation*}
Hence, $DV_rV_r^*D^{-1}$ is Hermitian. This means that $(DP^{1/2})(P^{1/2})^+D^{-1}$ is Hermitian by (24). On the other hand, we have
\begin{equation*}
    (P^{1/2})^+D^{-1}(DP^{1/2})(P^{1/2})^+D^{-1}=(P^{1/2})^+P^{1/2}(P^{1/2})^+D^{-1}=(P^{1/2})^+D^{-1}
\end{equation*}
 \begin{equation*}  
   DP^{1/2}((P^{1/2})^+D^{-1})DP^{1/2}=DP^{1/2}(P^{1/2})^+P^{1/2}=DP^{1/2}
    \end{equation*}
    \begin{equation*}
    (P^{1/2})^+D^{-1}(DP^{1/2})=(P^{1/2})^+P^{1/2}=V_r|\hat{\Lambda}_r|^{-1/2}|\hat{\Lambda}_r|^{1/2}V_r^*=V_rV_r^*
\end{equation*}
where $V_rV_r^*$ is Hermitian. By the definition of pseudo inverse $(DP^{1/2})^+=(P^{1/2})^+D^{-1}$ hence $(\Tilde{P}^{1/2})^+=W^*(DP^{1/2})^+=W^*(P^{1/2})^+D^{-1}$. Since $(P^{1/2})^+=V_r|\hat{\Lambda}_r|^{-1/2}V_r^*$, it is unitarily diagonalisable with real eigenvalues so it is Hermitian and similarly, $(\Tilde{P}^{1/2})^+$ is also Hermitian. Hence, $(\Tilde{P}^{1/2})^+=W^*(P^{1/2})^+D^{-1}=(W^*(P^{1/2})^+D^{-1})^*=D^{-*}(P^{1/2})^+W$. Since the derivation of (4) still holds for normal matrices, we have \begin{equation*}
    \begin{aligned}
        k=\|(\Tilde{A}^{1/2})^+\Tilde{E}(\Tilde{A}^{1/2})^+\|&\overset{(4)}{=}\|(\tilde{P}^{1/2})^+\Tilde{E}(\tilde{P}^{1/2})^+\|\\
        &=\|(W^*(P^{1/2})^+D^{-1})(DED^*)(D^{-*}(P^{1/2})^+W)\|\\
        &=\|W^*(P^{1/2})^+E(P^{1/2})^+W\|\\
        &=\|(P^{1/2})^+E(P^{1/2})^+\|\overset{(4)}{=}\|(A^{1/2})^+E(A^{1/2})^+\|
    \end{aligned}
\end{equation*}
\end{proof}
\begin{remark}
\textnormal{As shown in the proof of Theorem 3.1, the condition that $D^*D$ commutes with $V_rV_r^*$ is sufficient to imply $(DP^{1/2})^+=(P^{1/2})^+D^{-1}$, which means the pseudo inverse of $DP^{1/2}$ follows the reverse order law. This condition is also necessary because if  $(DP^{1/2})^+=(P^{1/2})^+D^{-1}$, then $DP^{1/2}(P^{1/2})^+D^{-1}=DV_rV_r^*D^{-1}$  must be Hermitian which means $DV_rV_r^*D^{-1}=(DV_rV_r^*D^{-1})^*=D^{-*}V_rV_r^*D^*$. Multiplying both side by $D^*$ on the left and $D$ on the right, we get $D^*DV_rV_r^*=V_rV_rD^*D$. More generally for any matrices $X, Y$, $(XY)^+=Y^+X^+$ if and only if $X^+X$ commutes with $YY^*$ and $YY^+$ commutes with $X^*X$, as suggested by [2, Theorem 3.1] and [9, Corollary 3.11].}
\end{remark}
We can now combine Theorem 3.1 with Theorem 2.1 to give a result extending [8, Corollary 2.2] and [10, Theorem 2.4] from the case $A$ being positive definite to $A$ being positive semi-definite and suggest the relative bounds of (1) and (2) for $A+E$ are the same as its congruence transformation $D(A+E)D^*$, under certain conditions.  \begin{corollary}
    Let $\Tilde{A}=DAD^*$ be positive semi-definite with rank $s\leq n$ and eigenvalues $\lambda_1\geq...\geq \lambda_s, \lambda_{s+1}=...=\lambda_n=0$. Let $\Tilde{A}+\Tilde{E}$ be also positive semi-definite with eigenvalues in decreasing order, where $\Tilde{E}=DED^*$.  If $k=\|(A^{1/2})^{+} E(A^{1/2})^{+}\|$, and $D$ is invertible with $D^*DV_rV_r^*=V_rV_r^*D^*D$ where $V$ is an eigenvector matrix of $A$ which is of rank $r$, we have for any $i\in \{1,...,s\},$
\begin{equation*}\lambda_{n-s+i}(\Tilde{A}+\Tilde{E})=\lambda_{n-s+i}(D(A+E)D^*)\leq \lambda_i+k\lambda_i
    \end{equation*}
and \begin{equation*}
    \lambda_i(\Tilde{A}+\Tilde{E})=\lambda_i(D(A+E)D^*) \geq \lambda_i -k\lambda_i
\end{equation*}\end{corollary}
\begin{proof}
We first apply Corollary 2.1.1 to $\Tilde{A}$ and $\Tilde{E}$ and obtain that for $i\in \{1,..,s\}$, \begin{equation*}\begin{aligned}
    \lambda_{n-s+i}(\Tilde{A}+\Tilde{E})=\lambda_{n-s+i}(D(A+E)D^*)\leq \lambda_i+\|(\Tilde{A}^{1/2})^+\Tilde{E}(\Tilde{A}^{1/2})^+\|\lambda_i
   \\ \lambda_i(\Tilde{A}+\Tilde{E})=\lambda_i(D(A+E)D^*) \geq \lambda_i -\|(\Tilde{A}^{1/2})^+\Tilde{E}(\Tilde{A}^{1/2})^+\|\lambda_i
\end{aligned}\end{equation*}
 Since $\Tilde{A}$ is positive semi-definite, its polar factor is itself. Since $D$ is invertible, $A=D^{-1}\Tilde{A}D^{-*}$ is positive semi-definite as for any vector $x$, $x^*Ax=x^*(D^{-1}\Tilde{A}D^{-*})x=(D^{-*}x)^*\Tilde{A}(D^{-*}x)\geq 0$. Hence, its polar factor is also itself. Since $\Tilde{A}=DAD^*$, the conditions for Theorem 3.1 are all satisfied, so $\|(A^{1/2})^+E(A^{1/2})^+\|=\|(\Tilde{A}^{1/2})^+\Tilde{E}(\Tilde{A}^{1/2})^+\|$. Hence, we can replace $\|(\Tilde{A}^{1/2})^+\Tilde{E}(\Tilde{A}^{1/2})^+\|$ by $k$ above and get the result. \end{proof}
In Theorem 3.1, when $A$ has full rank, the condition of $D^*D$ commuting with $V_rV_r^*$ becomes $D^*D$ commuting with $VV^*=I$ which holds for any $D$. Hence this extra constraint on $D$ compared to [8, Corollary 2.2] and [10, Theorem 2.4] vanishes so $D$ can be any invertible matrix. In Corollary 3.1.1, since $\Tilde{A}=DAD^*$ is known to be positive semi-definite, when $A$ is invertible,  it becomes positive definite so we recover [8, Corollary 2.2] and [10, Theorem 2.4]. When $r<n$, and the constraint tells us some structure that $D$ must have by the following observation.
\begin{observation*}
When $V$ is unitary and $r<n$, $D^*DV_rV_r^*=V_rV_r^*D^*D$ if and only if $D=U\Sigma W^*$ as its SVD where $W=VS$ for some permutation matrix $S$. 
\end{observation*}
\begin{proof}
 Let $k=\mbox{rank}(D^*D)$. Since $D^*D$ commutes with $V_rV_r^*=V\left[\begin{array}{cc}
     I_r &  \\
      & \mathbf{0}
 \end{array}\right]V^*$, by [7, Theorem 2.5.5], $D^*D$ can be diagonalised as $D^*D=V\hat{\Lambda} V^*$ where $\hat{\Lambda} $ is diagonal with eigenvalues of $D^*D$. Let $S$ be a permutation matrix such that  $\Lambda= S^*\hat{\Lambda}S$ is diagonal with eigenvalues of $D^*D$ in decreasing order, denoted as $\Lambda=\left[\begin{array}{cc}
    \Lambda_k  &  \\
      & \mathbf{0}
 \end{array}\right]$, hence $D^*D=V(S\Lambda S^*)V^*=W\Lambda W^*=W_k\Lambda_k W_k^*$ where $W=VS$ is unitary and $\Lambda_k >
 \mathbf{0}$. Now we attempt to construct the SVD of $D$. Let \begin{equation}
     D=DWW^*=DW\left[\begin{array}{cc}
         \Lambda_k^{-1/2} &  \\
          & I
     \end{array}\right]\left[\begin{array}{cc}
        \Lambda_k^{1/2}  &  \\
          & I
     \end{array}\right]\left[\begin{array}{cc}
         W_k^*  \\
         {W_k^\perp}^*
     \end{array}\right]
 \end{equation}
 Let $B=DW\left[\begin{array}{cc}
     \Lambda_k^{-1/2} &  \\
      & I
 \end{array}\right]=\left[\begin{array}{cc}
    B_k  & B_{n-k} \\
 \end{array}\right]$, then $B^*B=\left[\begin{array}{cc}
    B_k^*    \\
      B_{n-k}^* 
 \end{array}\right]\left[\begin{array}{cc}
    B_k  & B_{n-k} \\
 \end{array}\right]=\left[\begin{array}{cc}
    B_k^*B_k & B_k^*B_{n-k}  \\
    B_{n-k}^*B_k &  B_{n-k}^* B_{n-k}
 \end{array}\right]$. Since $W^*D^*DW^*=W^*W\Lambda W^*W=\left[\begin{array}{cc}
     \Lambda_k &  \\
      & \mathbf{0}
 \end{array}\right]$, we have \begin{equation*}
 \begin{aligned}
     B^*B&=\left[\begin{array}{cc}
     \Lambda_k^{-1/2} &  \\
      & I
 \end{array}\right]W^*D^*DW
\left[\begin{array}{cc}
     \Lambda_k^{-1/2} &  \\
      & I
 \end{array}\right]\\&=\left[\begin{array}{cc}
     \Lambda_k^{-1/2} &  \\
      & I
 \end{array}\right]\left[\begin{array}{cc}
     \Lambda_k &  \\
      & \mathbf{0}
 \end{array}\right] \left[\begin{array}{cc}
     \Lambda_k^{-1/2} &  \\
      & I
 \end{array}\right]\\&= \left[\begin{array}{cc}
     I_k &  \\
      & \mathbf{0}
 \end{array}\right] \end{aligned} \end{equation*}
Hence, $B^*_{n-k}B_{n-k}=\mathbf{0}$ which means $B_{n-k}=\mathbf{0}$, and $B_k^*B_k=I_k$. Take $U_k=B_k$ which is $n\times k$ orthonormal, then $B=\left[\begin{array}{cc}
    U_k  & \mathbf{0} \\
 \end{array}\right]$. We substitute it into (25) and get 

\begin{equation*}
     \begin{aligned}
       D&=\left[\begin{array}{cc}
          U_k  & \mathbf{0} \\
       \end{array}\right]\left[\begin{array}{cc}
    \Lambda_k^{1/2} &  \\
          & I
     \end{array}\right]\left[\begin{array}{cc}
         W_k^*  \\
          {W_k^\perp}^* 
     \end{array}\right]=U_k\Lambda_k^{1/2}W_k^*\\
     &=\left[\begin{array}{cc}
         U_k & U_k^\perp \\
     \end{array}\right]\left[\begin{array}{cc}
         \Lambda_k^{1/2} &  \\
          & \mathbf{0}
     \end{array}\right]\left[\begin{array}{cc}
         W_k^*  \\
          {W_k^\perp}^* 
     \end{array}\right]=U\Lambda^{1/2}W^*   \end{aligned}
     \end{equation*} 
In particular, take $\Lambda^{1/2}$ to be diagonal positive semi-definite with entries being square root of eigenvalues of $D^*D$ in decreasing order, and let $\Sigma=\Lambda^{1/2}$. Then $D=U\Sigma W^*$ is an SVD of $D$, where $W=VS$ for some permutation matrix $S$.

 On the other hand, if $D=U\Sigma (VS)^*$ as its SVD, \begin{equation*}D^*D=VS\Sigma U^*U\Sigma S^*V^*=VS\Sigma^2 S^* V^*=V\hat{\Lambda} V^*
 \end{equation*}
 Since $S$ is a permutation matrix , $\hat{\Lambda}= S\Sigma^2S^*$ is also diagonal. So $D^*D$ and $V_rV_r^*$ are simultaneously diagonalisable by $V$ so they must commute by [7, Theorem 1.3.21]. \end{proof}
 
 As pointed out in [8], the reason one care about congruence transformation is that it can be used to produce a matrix $DAD^*$ with entries and eigenvalues about the same order of magnitude while those of original matrix $A$ may be widely varying. This usage to extract the scaling out of a matrix is exploited in [3] and [11]. We will also make use of congruence transformation and Theorem 3.1 in Section 4.2.
\subsection{Comparison to Weyl's absolute bound}
We have seen several relative perturbation bounds taking the form of (1) and (2) stemming from Theorem 2.1. It is natural to ask how good  the relative bound in Theorem 2.1 can be and in particular, we would like to know under what circumstance the relative bound can be sharper than the Weyl's absolute  bound.

If we first assume that the Hermitian matrix $A$ has full rank, then the relative bound suggested by Theorem 2.1 coincides with the main theorem in [4], which is for $E$ being Hermitian, $i\in\{1,...,n\}$ ,  and $k=\|A^{-1/2}EA^{-1/2}\|\leq 1$, \begin{equation}
  |\lambda_i(A+E)-\lambda_i(A)|\leq k|\lambda_i(A)|
\end{equation}
where the orderings of $\lambda_i(A)$ and $ \lambda_i(A+E)$ are decreasing as before. On the other hand, the Weyl's absolute bound under the same context is for $i\in\{1,...,n\}$, \begin{equation}
    |\lambda_i(A+E)-\lambda_i(A)|\leq \|E\|
     \end{equation} 
To have (26) being sharper than (27) for the same index $i$ is equivalent to have $k|\lambda_i(A)|\leq \|E\|$, which will depend on the specific $i$ of interest. We will try to give a sufficient condition for it using a result of the Ostrowski's Theorem [7, Theorem 4.5.9] namely the Ostrowski's bound for multiplicative perturbation [5, Theorem 2.1] which we will state as follow:
\begin{theorem*}[Ostrowski's bound]
If $A$ and $DAD^*$ are Hermitian, where $D$ is non-singular, then for all $l\in \{1,...,n\}$, \begin{equation*}
    \frac{|\lambda_l(A)|}{\|(D^{*}D)^{-1}\|}\leq |\lambda_l(DAD^*)|\leq |\lambda_l(A)|\|D^*D\|
\end{equation*}
\end{theorem*} A proof can be found in [5, Theorem 2.1]. Using the above, we are able to present the following result in an attempt to give a sufficient condition for $k|\lambda_i(A)|\leq \|E\|$.
\begin{theorem}
    
Let $A$ be Hermitian non-singular with polar factor $P$, and $j'$ be any index such that $|\lambda_{j'}(P^{-1/2}EP^{-1/2})|=\max\limits_j|\lambda_j(P^{-1/2}EP^{-1/2})|$. For any Hermitian matrix $E$, if for any fixed $i\in \{1,...,n\}$, \begin{equation}
    \frac{|\lambda_i(A)|}{\min\limits_l|\lambda_l(A)|}|\lambda_{j'}(E)|\leq \|E\|
\end{equation}
then we have $k|\lambda_i(A)|\leq \|E\|$ where $k=\|A^{-1/2}EA^{-1/2}\|$. \end{theorem}
\begin{proof}
 Let $A=VDV^*$ be its spectral decomposition. Then $P=V|D|V^*$ and $P^{-1/2}=V|D|^{-1/2}V^*$, so $P^{-1/2}$ is Hermitian. As $E$ is Hermitian, so is $P^{-1/2}EP^{-1/2}$. Therefore, $|\lambda_{j'}(P^{-1/2}EP^{-1/2})|=\max\limits_j|\lambda_j(P^{-1/2}EP^{-1/2})|=\|P^{-1/2}EP^{-1/2}\|$. We can apply the Ostrowski's bound to $P^{-1/2}EP^{-1/2}$ and $E=P^{1/2}(P^{-1/2}EP^{-1/2})(P^{1/2})^*$ with the index being $j'$,  and obtain that
\begin{equation}
\begin{aligned}
    |\lambda_{j'}(E)|&\geq \frac{|\lambda_{j'}(P^{-1/2}EP^{-1/2})|}{\|(P^{1/2}P^{1/2})^{-1}\|}\\&=\frac{\|P^{-1/2}EP^{-1/2}\|}{\|P^{-1}\|}\\
    &\overset{(4)}{=}\frac{\|A^{-1/2}EA^{-1/2}\|}{\|A^{-1}\|}=k\min\limits_l|\lambda_l(A)|
    \end{aligned}
\end{equation}
where the last equality uses that $\|A^{-1}\|=1/\min\limits_l|\lambda_l(A)|$ since $A^{-1}=VD^{-1}V^*$. We substitute (29) into (28) which is given, and obtain that \begin{equation*}
\begin{aligned}
    \|E\|&\geq |\lambda_{j'}(E)|\frac{|\lambda_i(A)|}{\min\limits_l|\lambda_l(A)|}\\
    &\geq k\min\limits_l|\lambda_l(A)|\frac{|\lambda_i(A)|}{\min\limits_l|\lambda_l(A)|}\\&=k|\lambda_i(A)|
     \end{aligned}
     \end{equation*}\end{proof}  
\begin{remark} \textnormal{Because $\|E\|=\max\limits_j|\lambda_j(E)|=|\lambda_{j^*}(E)|$, we can only expect condition (28) to hold for more $i\in\{1,...,n\}$ besides $i'$ where $|\lambda_{i'}(A)|=\min\limits_l|\lambda_l(A)|$ when $j'$ are $j^*$ are genuine different indices such that $|\lambda_{j'}(E)|<|\lambda_{j^*}(E)|$. This limits the scope of application for Theorem 3.2.}
\end{remark} 
 
 Theorem 3.2 gives a general sense of when the relative bound in (26) is possibly sharper than (27). When we are looking at $\lambda_i(A+E)$ at index $i$ such that the corresponding $|\lambda_i(A)|$ is closer to $\min\limits_l|\lambda_l(A)|$, it is more likely to have $ k|\lambda_i(A)|\leq \|E\|$ because the ratio between $|\lambda_i(A)|$ and $\min\limits_l|\lambda_l(A)|$ is more likely to be smaller than the ratio between $\|E\|$ and $|\lambda_{j'}(E)|$ where $j'$ is defined as before,  so (28) is satisfied and we can apply Theorem 3.2. This can be illustrated as below:

\begin{theorem}
    Let $A$ be Hermitian non-singular and $E$ be any Hermitian matrix, if $k=\|A^{-1/2}EA^{-1/2}\|$, then there exists some index $i\in \{1,...,n\}$ such that \begin{equation*}
        |\lambda_i(A+E)-\lambda_i(A)|\leq k|\lambda_i(A)|\leq\|E\|
    \end{equation*}
\end{theorem}
\begin{proof}
    Take $i\in\{1,...,n\}$ such that $|\lambda_i(A)|=\min\limits_l|\lambda_l(A)|$. Since  $\|E\|=\max\limits_j|\lambda_j(E)|$ because $E$ is Hermitian, for any $j'\in \{1,...,n\}$, \begin{equation*}
         \frac{|\lambda_i(A)|}{\min\limits_l|\lambda_l(A)|}|\lambda_{j'}(E)|=|\lambda_{j'}(E)|\leq \|E\|
    \end{equation*}
So (28) is satisfied. By Theorem 3.2, we have $|\lambda_i(A+E)-\lambda_i(A)|\leq k|\lambda_i(A)|\leq \|E\|$.

\end{proof}


 To conclude, it may depend on the index $i\in \{1,...,n\}$ of interest to have whether $ k|\lambda_i(A)|\leq \|E\|$ or the contrary, but Theorem 3.3 ensures that there always exists some index $i\in \{1,...,n\}$  such that the relative bound in (26) is sharper than the Weyl's bound in (27).

More generally when $A$ has rank $r\leq n$ in Theorem 2.1, we want to compare \begin{equation}
    \lambda_{n-r+i}(A+E)\leq \lambda_i(A)+k|\lambda_i(A)|
\end{equation}
 with its corresponding Weyl's bound $\lambda_{n-r+i}(A+E)\leq \lambda_{n-r+i}(A)+\|E\|$,  and \begin{equation}
\lambda_i(A+E)\geq \lambda_i(A)-k|\lambda_i(A)|
 \end{equation} with its corresponding Weyl's bound $\lambda_i(A+E)\geq \lambda_i(A)-\|E\|$, for $i\in \{1,...,r\}$, when $A$ is potentially singular and $k=\|(A^{1/2})^+E(A^{1/2})^+\|$. 
 We can give a sufficient condition for the relative bounds in (30) and (31) being sharper than their corresponding Weyl's bounds by mimicking the argument in Theorem 3.2, although it involves more terms and the condition becomes less likely to achieve for a matrix with rank $r$, as $r$ decreases further away from $n$.   \begin{theorem}
    Let $A$ be Hermitian with rank $r\leq n$ with polar factor $P$, and $j'$ be any index such that $|\lambda_{j'}((P^{1/2})^+E(P^{1/2})^+)|=\max\limits_{j }|\lambda_j((P^{1/2})^+E(P^{1/2})^+)|$ where the eigenvalues of $(P^{1/2})^+E(P^{1/2})^+$ and $A$ are arranged in decreasing order with any zero eigenvalues occurring last.  Let $E$ be Hermitian. For any fixed
     $i\in\{1,...,r\}$, if \begin{equation}
\lambda_i(A)-\lambda_{n-r+i}(A)+\frac{\max \{|\lambda_{j'}(E)|, |\lambda_{n-r+j'}(E)| \}}{\min\limits_{l: \lambda_l(A)\neq 0}|\lambda_l(A)|}|\lambda_i(A)|\leq \|E\|
 \end{equation} 
 then $\lambda_{i}(A)+k|\lambda_i(A)|\leq \lambda_{n-r+i}(A)+\|E\|$ and $\lambda_{i}(A)-k|\lambda_i(A)|\geq \lambda_{i}(A)-\|E\|$, where $k=\|(A^{1/2})^+E(A^{1/2})^+\|$. \end{theorem}
\begin{proof}
Let $A=VDV^*=V_rD_rV_r^*$ be its spectral decomposition, then $P=V_r|D_r|V_r^*$, and $(P^{1/2})^+=(V_r|D_r|^{1/2}V_r^*)^+=V_r|D_r|^{-1/2}V_r^*$ is Hermitian. Since $(P^{1/2})^+E(P^{1/2})^+$ is Hermitian because $(P^{1/2})^+$ and $E$ are Hermitian, we have\begin{equation*}
   k=\|(A^{1/2})^+E(A^{1/2})^+\|\overset{(4)}{=}\|(P^{1/2})^+E(P^{1/2})^+\|=|\lambda_{j'}((P^{1/2})^+E(P^{1/2})^+)|  
   \end{equation*}
   Since $\mbox{rank}((P^{1/2})^+E(P^{1/2})^+)\leq \mbox{rank}((P^{1/2})^+)=r$,  the index $j'\in \{1,...,r\}$, because $\lambda_{j}((P^{1/2})^+E(P^{1/2})^+)=0$ for any $j>r$ by the specified ordering of eigenvalues of $(P^{1/2})^+E(P^{1/2})^+$, assuming $(P^{1/2})^+E(P^{1/2})^+\neq \mathbf{0}$.\footnote{If $(P^{1/2})^+E(P^{1/2})^+=V_r|D_r|^{-1/2}V_r^*EV_r|D_r|^{-1/2}V_r^*=\mathbf{0}$, multiplying both sides by $|D_r|^{1/2}V_r^*$ on the left and $V_r|D_r|^{1/2}$ on the right we get $V_r^*EV_r=\mathbf{0}$. We can still take $j'\in \{1,...,r\}$ since all the eigenvalues are zero and the rest of the deviation will all hold true. } Then for such $j'\in \{1,...,r\}$, using $\mbox{eig}(XY)=\mbox{eig}(YX)$ [7, Theorem 1.3.22],
\begin{equation}
\begin{aligned}
   k= \|(P^{1/2})^+E(P^{1/2})^+\|&=|\lambda_{j'}((P^{1/2})^+E(P^{1/2})^+)|\\
    &=|\lambda_{j'}(\underbrace{V_r}_{X}\underbrace{|D_r|^{-1/2}V_r^*EV_r|D_r|^{-1/2}V_r^*}_{Y})| \\
    &=|\lambda_{j'}(|D_r|^{-1/2}V_r^*EV_r|D_r|^{-1/2}V_r^*V_r)| \\ &=|\lambda_{j'}(|D_r|^{-1/2}V_r^*EV_r|D_r|^{-1/2})|  \\
        \end{aligned}
\end{equation}
On the other hand, since $V_r^*EV_r=|D_r
|^{1/2}(|D_r|^{-1/2}V_r^*EV_r|D_r|^{-1/2})|D_r|^{1/2}$ where $|D_r|^{1/2}$ is Hermitian non-singular, we can apply the Ostrowski's bound to $V_r^*EV_r$  $|D_r|^{-1/2}V_r^*EV_r|D_r|^{-1/2}$ at index $j'\in \{1,...,r\}$, and obtain  
\begin{equation}
       |\lambda_{j'}(V_r^*EV_r)|\geq \frac{|\lambda_{j'}(|D_r|^{-1/2}V_r^*EV_r|D_r|^{-1/2})|}{\|(|D_r|^{1/2}|D_r|^{1/2})^{-1}\|}
       =\frac{|\lambda_{j'}(|D_r|^{-1/2}V_r^*EV_r|D_r|^{-1/2})|}{\||D_r|^{-1}\|}
       \end{equation}
We substitute (33) and that $\||D_r|^{-1}\|=1/\min\limits_{l: \lambda_l(A)\neq 0}|\lambda_l(A)|$ into (34), and obtain \begin{equation} 
    |\lambda_{j'}(V_r^*EV_r)|\geq \|(P^{1/2})^+E(P^{1/2})^+\|\min\limits_{l: \lambda_l(A)\neq 0}|\lambda_l(A)|=k\min\limits_{l: \lambda_l(A)\neq 0}|\lambda_l(A)|
    \end{equation}
By [7, Theorem 4.3.28], and (7) but with $E$, since $j'\in \{1,...,r\}$, \begin{equation*}
\lambda_{n-r+j'}(E)=\lambda_{n-r+j'}(V^*EV)\leq \lambda_{j'}(V_r^*EV_r)\leq\lambda_{j'}(V^*EV)=\lambda_{j'}(E)
   \end{equation*} which means $|\lambda_{j'}(V_r^*EV_r)|\leq \max\{|\lambda_{j'}(E)|, |\lambda_{n-r+j'}(E)| \} $. Then we substitute this and (35) into (32) which is given and get\begin{equation*}
   \begin{aligned}
       \|E\|&\geq \lambda_i(A)-\lambda_{n-r+i}(A)+\frac{\max \{|\lambda_{j'}(E)|, |\lambda_{n-r+j'}(E)| \}}{\min\limits_{l: \lambda_l(A)\neq 0}|\lambda_l(A)|}|\lambda_i(A)| \\
       &\geq\lambda_i(A)-\lambda_{n-r+i}(A)+\frac{|\lambda_{j'}(V_r^*EV_r)}{\min\limits_{l: \lambda_l(A)\neq 0}|\lambda_l(A)|}|\lambda_i(A)|  \\
       &\overset{(35)}{\geq}\lambda_i(A)-\lambda_{n-r+i}(A)+k|\lambda_i(A)|        \end{aligned}      
       \end{equation*}
       which means that $\lambda_{i}(A)+k|\lambda_i(A)|\leq \lambda_{n-r+i}(A)+\|E\|$. Also, since $\lambda_{n-r+i}(A)\leq \lambda_i(A)$, we have $k|\lambda_i(A)|\leq \|E\|$ so $\lambda_i(A)-k|\lambda_i(A)|\geq \lambda_i(A)-\|E\|$. As a result, the relative bounds in (30) and (31) are tighter than their corresponding Weyl's bounds. \end{proof}
   
     Theorem 3.4 generalises Theorem 3.2 to $A$ having rank $r\leq n$. When $A$ is of full rank, we substitute $r=n$ into Theorem 3.4 and replace any pseudo inverse with normal inverse, then we will recover Theorem 3.2. We will illustrate when Theorem 3.4 could be useful in the next result which is also an extension of Theorem 3.3.
    
       \begin{corollary}
           Let $A$ be Hermitian of rank $r\leq n$ with eigenvalues $\lambda_1\geq...\geq \lambda_r, \lambda_{r+1}=...=\lambda_n=0$. Let $E$ be Hermitian, and $k=\|(A^{1/2})^+E(A^{1/2})^+\|$. If the eigenvalue with the smallest non-zero absolute value of $A$ has at least $n-r+1$ algebraic multiplicity, then there exists some $i\in \{1,...,r\}$ such that 
\begin{equation*}
\begin{array}{cc}
\lambda_{i}+k|\lambda_i|\leq \lambda_{n-r+i}+\|E\|, &  \lambda_i-k\|\lambda_i\|\geq \lambda_i-\|E\|\\
\end{array}
    \end{equation*} 
       \end{corollary}
       \begin{proof}
           Take $i=\min\{j\in \{1,...,r\}: |\lambda_j|=\min\limits_{l:\lambda_l\neq 0}|\lambda_l|\}$. Since there are at least $n-r+1$ copies of $\lambda_i$ among the eigenvalues of $A$, by the ordering specified, $\lambda_{n-r+i}=\lambda_i$. Also, $|\lambda_i|=\min\limits_{l:\lambda_l\neq 0}|\lambda_l|$ by the definition of $i$. Hence, for any $j'\in \{1,...,n\}$,
        \begin{equation*}
        \begin{aligned}
\lambda_i-\lambda_{n-r+i}+\frac{\max \{|\lambda_{j'}(E)|, |\lambda_{n-r+j'}(E)| \}}{\min\limits_{l: \lambda_l\neq 0}|\lambda_l|}|\lambda_i|&=\max \{|\lambda_{j'}(E)|, |\lambda_{n-r+j'}(E)|\} \\ 
&\leq \max\limits_{l'}|\lambda_{l'}(E)|=\|E\|\end{aligned}
        \end{equation*}
as $E$ is Hermitian, so (32) is satisfied for such $i\in \{1,...,r\}$. By Theorem 3.4, we have $\lambda_{i}+k|\lambda_i|\leq \lambda_{n-r+i}+\|E\|$, which gives $\lambda_i-k|\lambda_i|\geq \lambda_i-\|E\|$ as well. As a result, the relative bounds in (30) and (31) are sharper than their corresponding Weyl's bounds for such index $i$. \end{proof}
In particular, when $A$ has full rank, the eigenvalue with the smallest absolute value of $A$ always has an algebraic multiplicity of at least $1$. In this case, the above result gives Theorem 3.3. As a result, Corollary 3.4.1 provides some justification that in some cases we should consider the relative bounds of (1) and (2) instead of their corresponding  Weyl's bounds.




==> contents.tex/Chapter_3.tex <==

\section{Relative bounds for singular values}
 Theorem 2.1 can be utilised to derive relative bounds on singular values of general matrices because singular values and eigenvalues are closely related. We will follow the same strategy as the proof of [5, Theorem 3.3], which is to consider the related Jordan-Wielandt matrix 
 such that its eigenvalues includes all the singular values of interest by [7, Theorem 7.3.3] and then obtain the following result that is structurally similar to [4, Theorem 3.1], but also applicable to singular values of more general matrices, because Theorem 2.1 can be applied to Hermitian matrices without full rank. We will also see that the relative bound for singular values below involve a constant $k=\|S^+ES^+\|$ where $S$ can be thought of as a pseudo $A^{1/2}$, resembling Theorem 2.1 for eigenvalues. We will first let $m\geq n$ for definiteness.
 
 \begin{theorem}
Let $A$ be a $m\times n$ matrix of rank $r$ with SVD $A=U\Sigma V^*=U_r\Sigma_r V_r^*$. Let $E$ be any $m\times n$ matrix and $S^+=V_r\Sigma_r^{-1/2} U_r^*$. If $k=\|S^+ES^+\|\leq 1$, then \begin{equation}
    \sigma_{m+n-2r+i}(A+E)\leq \sigma_i(A)+k\sigma_i(A)
\end{equation} for any $i\in \{1,...,2r-m\}$, and also\begin{equation}
    \sigma_i(A+E)\geq \sigma_i(A)-k\sigma_i(A) 
\end{equation} for any $i\in \{1,...,r\}$.
\end{theorem}
\begin{proof}
 Following the idea in [5, Theorem 3.3], let $\Tilde{A}=\left[\begin{array}{cc}
     & A \\
   A^*  & 
\end{array}\right]$, $\Tilde{E}=\left[\begin{array}{cc}
     & E \\
  E^*   & 
\end{array}\right]$ and $\Tilde{A}+\Tilde{E}=\left[\begin{array}{cc}
     &  A+E\\
   (A+E)^*  & 
\end{array}\right]$ which are all Hermitian $(m+n)\times (m+n)$ matrices. We first want to show (36). Using [7, Theorem 7.3.3], \begin{equation*}
\Tilde{A}=\left[\begin{array}{cc}
         & A \\
      A^*   & 
    \end{array}\right]=\left[\begin{array}{ccc}
       \frac{1}{\sqrt{2}}U  &  -\frac{1}{\sqrt{2}}U & U^\perp\\
  \frac{1}{\sqrt{2}}V &   \frac{1}{\sqrt{2}}V & \mathbf{0}    \end{array}\right] \left[\begin{array}{ccc}
     \Sigma  &  & \\
       & -\Sigma & \\
     &  & \mathbf{0}
  \end{array}\right]\left[\begin{array}{ccc}
\frac{1}{\sqrt{2}}U^* & \frac{1}{\sqrt{2}}V^*\\
-\frac{1}{\sqrt{2}}U^* & \frac{1}{\sqrt{2}}V^*  \\
{U^\perp}^* & \mathbf{0} \\ \end{array}\right]
\end{equation*} is its unitary diagonalisation and has eigenvalues $\sigma_1(A),..., \sigma_n(A), -\sigma_1(A),...,-\sigma_n(A)$ together with $m-n$ copies of zeros. Since $A$ has rank $r$, $\Tilde{A}$ has rank $2r$. Our aim is to apply Theorem 2.1 to $\Tilde{A}$ and $\tilde{E}$ suggesting if we show that $\|(\Tilde{A}^{1/2})^+\Tilde{E}(\Tilde{A}^{1/2})^+\|\leq 1$, then for any $i\in \{1,...,2r\},$ \begin{equation}
\begin{aligned}
    \lambda_{m+n-2r+i}(\Tilde{A}+\Tilde{E})&\leq \lambda_i(\Tilde{A})+\|(\Tilde{A}^{1/2})^+\Tilde{E}(\Tilde{A}^{1/2})^+\||\lambda_i(\Tilde{A})|\\
    &\overset{(4)}{=}\lambda_i(\Tilde{A})+\|(\Tilde{P}^{1/2})^+\Tilde{E}(\Tilde{P}^{1/2})^+\||\lambda_i(\Tilde{A})|\end{aligned}
\end{equation}
where $\Tilde{P}$ is the polar factor of $\Tilde{A}$. By [7, Theorem 7.3.1] it can be expressed as \begin{equation*}
    \Tilde{P}=(\Tilde{A}^*\Tilde{A})^{1/2}=\left[\begin{array}{ccc}
       \frac{1}{\sqrt{2}}U  &  -\frac{1}{\sqrt{2}}U & U^\perp\\
  \frac{1}{\sqrt{2}}V &   \frac{1}{\sqrt{2}}V & \mathbf{0}    \end{array}\right] \left[\begin{array}{ccc}
     \Sigma  &  & \\
       & \Sigma & \\
     &  & \mathbf{0}
  \end{array}\right]\left[\begin{array}{ccc}
\frac{1}{\sqrt{2}}U^* & \frac{1}{\sqrt{2}}V^*\\
-\frac{1}{\sqrt{2}}U^* & \frac{1}{\sqrt{2}}V^*  \\
{U^\perp}^* & \mathbf{0} \\ \end{array}\right]\end{equation*}

As a result, \begin{equation*}
\begin{aligned}
    \Tilde{P}^{1/2}&=\left[\begin{array}{ccc}
       \frac{1}{\sqrt{2}}U  &  -\frac{1}{\sqrt{2}}U & U^\perp\\
  \frac{1}{\sqrt{2}}V &   \frac{1}{\sqrt{2}}V & \mathbf{0}    \end{array}\right] \left[\begin{array}{ccc}
     \Sigma^{1/2}  &  & \\
       & \Sigma^{1/2} & \\
     &  & \mathbf{0}
  \end{array}\right]\left[\begin{array}{ccc}
\frac{1}{\sqrt{2}}U^* & \frac{1}{\sqrt{2}}V^*\\
-\frac{1}{\sqrt{2}}U^* & \frac{1}{\sqrt{2}}V^*  \\
{U^\perp}^* & \mathbf{0} \\ \end{array}\right] \\
&=\left[\begin{array}{ccc}
       \frac{1}{\sqrt{2}}U\Sigma^{1/2}  &  -\frac{1}{\sqrt{2}}U\Sigma^{1/2} & \mathbf{0}\\
  \frac{1}{\sqrt{2}}V\Sigma^{1/2} &   \frac{1}{\sqrt{2}}V\Sigma^{1/2} & \mathbf{0}    \end{array}\right]\left[\begin{array}{ccc}
\frac{1}{\sqrt{2}}U^* & \frac{1}{\sqrt{2}}V^*\\
-\frac{1}{\sqrt{2}}U^* & \frac{1}{\sqrt{2}}V^*  \\
{U^\perp}^* & \mathbf{0} \\ \end{array}\right]\\
&=\left[\begin{array}{cc}
   U\Sigma^{1/2}U^*  &  \\
     & V\Sigma^{1/2}V^*
\end{array}\right]=\left[\begin{array}{cc}
   U_r\Sigma_r^{1/2}U_r^*  &  \\
     & V_r\Sigma_r^{1/2}V_r^*
\end{array}\right]\end{aligned}
\end{equation*}
because there are $r$ non-zero diagonal entries in $\Sigma^{1/2}$. As shown similarly in the proof of Theorem 2.4, since it $\Tilde{P}^{1/2}$ is a block diagonal matrix, its pseudo inverse is \begin{equation*}
  (\Tilde{P}^{1/2})^+ =\left[\begin{array}{cc}
   (U_r\Sigma_r^{1/2}U_r^* )^+ &  \\
     & (V_r\Sigma_r^{1/2}V_r^*)^+
\end{array}\right] =\left[\begin{array}{cc}
   U_r\Sigma_r^{-1/2}U_r^*  &  \\
     & V_r\Sigma_r^{-1/2}V_r^*
\end{array}\right]\end{equation*}
Substituting this into $(\Tilde{P}^{1/2})^+\Tilde{E}(\Tilde{P}^{1/2})^+$, we obtain
\begin{equation*}\begin{aligned}
   (\Tilde{P}^{1/2})^+\Tilde{E}(\Tilde{P}^{1/2})^+&=\left[\begin{array}{cc}
   U_r\Sigma_r^{-1/2}U_r^*  &  \\
     & V_r\Sigma_r^{-1/2}V_r^*
\end{array}\right] \left[\begin{array}{cc}
     & E \\
  E^*   & 
\end{array}\right](\Tilde{P}^{1/2})^+  \\
&=\left[\begin{array}{cc}
    &U_r\Sigma_r^{-1/2}U_r^* E\\
V_r\Sigma_r^{-1/2}V_r^*E^* & 
\end{array}\right]\left[\begin{array}{cc}
   U_r\Sigma_r^{-1/2}U_r^*  &  \\
     & V_r\Sigma_r^{-1/2}V_r^*
\end{array}\right]\\
&=\left[\begin{array}{cc}
    &U_r\Sigma_r^{-1/2}U_r^* E V_r\Sigma_r^{-1/2}V_r^*\\
(U_r\Sigma_r^{-1/2}U_r^* E V_r\Sigma_r^{-1/2}V_r^*)^*& 
\end{array}\right]
\end{aligned}
    \end{equation*}
    which is the Jordan-Wielandt matrix of $U_r\Sigma_r^{-1/2}U_r^* E V_r\Sigma_r^{-1/2}V_r^*$ so its eigenvalues are the singular values of $U_r\Sigma_r^{-1/2}U_r^* E V_r\Sigma_r^{-1/2}V_r^*$, their negations and zeros. Recall $U$ is $m\times n$ orthonormal, $V$ is $n\times n$ unitary in the SVD of $A$, hence for any $n\times n$ matrix $X$, $\|UXV^*\|=\|X\|=\|X^*\|=\|UX^*V^*\|=\|(UX^*V^*)^*\|=\|VXU^*\|$.  So
 \begin{equation}
       \begin{aligned}
            \|(\Tilde{P}^{1/2})^+\Tilde{E}(\Tilde{P}^{1/2})^+\|&=\max\limits_i|\lambda_i((\Tilde{P}^{1/2})^+\Tilde{E}(\Tilde{P}^{1/2})^+)|\\
            &=\sigma_1(U_r\Sigma_r^{-1/2}U_r^* E V_r\Sigma_r^{-1/2}V_r^*) \\            &=\|U_r\Sigma_r^{-1/2}U_r^* E V_r\Sigma_r^{-1/2}V_r^* \| \\
            &=\|U\underbrace{\left[\begin{array}{cc}
\Sigma_r^{-1/2}&  \\
                 & \mathbf{0}
            \end{array}\right]U^* E V\left[\begin{array}{cc}
\Sigma_r^{-1/2} &  \\
                 & \mathbf{0}
            \end{array}\right]}_{X}V^* \|      \\
            &=\|\left[\begin{array}{cc}
\Sigma_r^{-1/2}&  \\
                 & \mathbf{0}
            \end{array}\right]U^* E V\left[\begin{array}{cc}
\Sigma_r^{-1/2} &  \\
                 & \mathbf{0}
            \end{array}\right] \|   \\
            &=\|V\left[\begin{array}{cc}
\Sigma_r^{-1/2}&  \\
                 & \mathbf{0}
            \end{array}\right]U^* E V\left[\begin{array}{cc}
\Sigma_r^{-1/2} &  \\
                 & \mathbf{0}
            \end{array}\right]U^*\|  \\
            &=\|V_r\Sigma_r^{-1/2} U_r^* E V_r\Sigma_r^{-1/2}U_r^* \| =\|S^+ES^+\|=k          
            \end{aligned}   \end{equation}
 Therefore, since $\|(\Tilde{A}^{1/2})^+\Tilde{E}(\Tilde{A}^{1/2})^+\|\overset{(4)}{=}\|(\Tilde{P}^{1/2})^+\Tilde{E}(\Tilde{P}^{1/2})^+\|=k\leq 1$, by (1) in Theorem 2.1, we have (38) which is for $i\in \{1,...,2r\}$,\begin{equation}
     \lambda_{m+n-2r+i}(\Tilde{A}+\Tilde{E})\leq \lambda_i(\Tilde{A})+k|\lambda_i(\Tilde{A})|
     \end{equation}    where $\lambda_1(\Tilde{A})\geq...\geq \lambda_{2r}(\Tilde{A}), \lambda_{2r+1}(\Tilde{A})=...=\lambda_{m+n}(\Tilde{A})=0$ and the eigenvalues of $\Tilde{A}+\Tilde{E}$ are in decreasing order, as in Theorem 2.1. Since the eigenvalues of $\Tilde{A}+\Tilde{E}$ are $\sigma_1(A+E),...,\sigma_n(A+E), 0,..,0, -\sigma_n(A+E),...,-\sigma_1(A+E)$, for $m+n-2r+i\leq n$ which is $i\leq 2r-m$, $\lambda_{m+n-2r+i}(\Tilde{A}+\Tilde{E})=\sigma_{m+n-2r+i}(A+E)$. The eigenvalues of $\Tilde{A}$ in the ordering specified before are $\sigma_1(A),...,\sigma_r(A), -\sigma_r(A),...,-\sigma_1(A), 0,...,0$. For $i\leq r$, we have $\lambda_i(\Tilde{A})=\sigma_i(A)$. Since $r=\mbox{rank}(A)\leq m$, $2r-m\leq r$, so for $i\leq 2r-m$, we have $m+n-2r+i\leq n$ and $i\leq r$, which gives $\lambda_{m+n-2r+i}(\Tilde{A}+\Tilde{E})=\sigma_{m+n-2r+i}(A+E)$ and $\lambda_i(\Tilde{A})=\sigma_i(A)$. Substituting them into (40), we get  $ \sigma_{m+n-2r+i}(A+E)\leq \sigma_i(A)+k\sigma_i(A)$ which is (36), for $i\in \{1,...,2r-m\}.$

 On the other hand to show (37), we apply (2) in Theorem 2.1 to $\Tilde{A}$ and $\Tilde{E}$ since $\|(\Tilde{A}^{1/2})^+\Tilde{E}(\Tilde{A}^{1/2})^+\|\leq 1$, and obtain for $i\in\{1,...,2r\}$ \begin{equation}
     \lambda_i(\Tilde{A}+\Tilde{E})\geq \lambda_i(\Tilde{A})-k|\lambda_i(\Tilde{A})|
 \end{equation}
  When $i\leq r$, $\lambda_i(\Tilde{A})=\sigma_i(A)$ and when $i\leq n$, $\lambda_i(\Tilde{A}+\Tilde{E})=\sigma_i(A+E)$. Since $r\leq n$ , when $i\leq r$, we have both. Therefore when $i\leq r$, substituting them into (41), we get 
  $\sigma_i(A+E)\geq \sigma_i(A)-k\sigma_i(A)$ which is (37) for $i\in \{1,...,r\}$. 
 \end{proof}
 \begin{remark}
     \textnormal{Since $S^+=V_r\Sigma_r^{-1/2}U_r^*$, $S=U_r \Sigma_r^{1/2}V_r^*$. Then
$S^*S=V_r\Sigma_r^{1/2}U_r^*U_r\Sigma_r^{1/2}V_r^*=V_r\Sigma_rV_r^*$ which is the right polar factor of the tall matrix $A$ by [7, Theorem 7.3.1]. In the case that $A$ is normal, $A^{1/2}=VD^{1/2}V^*$ and $(A^{1/2})^*A^{1/2}=V(D^{1/2})^*D^{1/2}V^*=V|D|V^*$ which is the polar factor of $A$. Therefore, such $S$ can be regarded as pseudo $A^{1/2}$ when $A$ is $m\times n$ where $m\geq n$, because it exhibits a same property of  $A^{1/2}$ when $A$ is normal, although we do not have $S^2=A$.  We can also consider the case $A$ has more columns than rows using Theorem 4.1.}
 \end{remark}
 \begin{corollary}
Let $A$ be a $n \times m$ matrix of rank $r$ with SVD $A=U\Sigma V^*=U_r\Sigma_r V_r^*$. Let $E$ be any $n\times m$ matrix and $S^+=V_r\Sigma_r^{-1/2}U_r^*$. If $k=\|S^+ES^+\|\leq 1$, then \begin{equation*}
    \sigma_{m+n-2r+i}(A+E)\leq \sigma_i(A)+k\sigma_i(A)
\end{equation*} for any $i\in \{1,...,2r-m\}$, and also\begin{equation*}
    \sigma_i(A+E)\geq \sigma_i(A)-k\sigma_i(A) 
\end{equation*} for any $i\in \{1,...,r\}$ \end{corollary}
\begin{proof}
    Since $A=U\Sigma V^*$  where $U$ is $n \times n$ unitary and $V$ is $m\times n$ orthonormal, $A^*=V\Sigma U^*$ as its SVD and it is of size $m\times n$ where $m\geq n$ and rank $r$. Since $k\leq 1$, $\|(S^+)^*E^*(S^+)^*\|=\|(S^+ES^+)^*\|=\|S^+ES^+\|\leq 1$, where $(S^+)^*=U_r\Sigma_r^{-1/2} V_r^*$. We apply Theorem 4.1 to $A^*$ and $E^*$, and obtain $ \sigma_{m+n-2r+i}(A^*+E^*)\leq \sigma_i(A^*)+\|(S^+)^*E^*(S^+)^*\|\sigma_i(A^*)$
for $i\in \{1,...,2r-m\}$, and also
    $\sigma_i(A^*+E^*)\geq \sigma_i(A^*)-\|(S^+)^*E^*(S^+)^*\|\sigma_i(A^*)$
for $i\in \{1,...,r\}$.  Since any singular value is invariant under matrix transpose and $\|(S^+)^*E^*(S^+)^*\|=k$, we get $\sigma_{m+n-2r+i}(A+E)\leq \sigma_i(A)+k\sigma_i(A)$
 for $i\in \{1,...,2r-m\}$, and $\sigma_i(A+E)\geq \sigma_i(A)-k\sigma_i(A)$ for $i\in \{1,...,r\}$ 
\end{proof}

As in Theorem 4.1, $S=U_r\Sigma_r^{1/2}V_r^*$ can be regarded as a pseudo $A^{1/2}$. This is because $SS^*=U_r\Sigma_r^{1/2}V_r^*V_r\Sigma_r^{1/2}U_r^*=U_r\Sigma_rU_r^*$ which is the left polar factor of the wide matrix $A$ by [7, Theorem 7.3.1], whereas in the case that $A$ is normal, $A^{1/2}(A^{1/2})^*=VD^{1/2}(D^{1/2})^*V^*=V|D|V^*$ which is the polar factor of $A$. Hence, such $S$ has a same property as $A^{1/2}$ when $A$ is normal. 

Combining Theorem 4.1 and Corollary 4.1.1, we can drop the assumption that $m\geq n$, and conclude that for any $m\times n$ matrix $A=U_r\Sigma_rV_r^*$ of rank $r$ and $m\times n$ matrix $E$, we always have (36) for any  $i\in \{1,...,2r-\max\{m,n\}\}$, and (37) for any $i\in \{1,...,r\}$, given that $k=\|S^+ES^+\|\leq 1$ where $S=U_r\Sigma_r^{1/2}V_r^*$ is regraded as a pseudo $A^{1/2}$. When $m=n$, $A$ is a square matrix and has both a left and right polar decomposition as $A=P_1Q=QP_2$ by [7, Theorem 7.3.1]. The following result illustrates that we can replace $k=\|S^+ES^+\|$ by an expression in terms of the polar factors $P_1, P_2$ of $A$. \begin{corollary}
    Let $A$ be a $n \times n$ matrix with left and right polar factorisation $A=P_1Q=QP_2$, and $E$ be any $n\times n$ matrix. If $k=\|(P_1^{1/2})^+E(P_2^{1/2})^+\|\leq 1$, then \begin{equation}
    \sigma_{2n-2r+i}(A+E)\leq \sigma_i(A)+ k\sigma_i(A)
\end{equation}
for any $i\in \{1,..., 2r-n\}$, and \begin{equation}
    \sigma_i(A+E)\geq \sigma_i(A)-k\sigma_i(A)
\end{equation}
for any $i\in \{1,..., r\}.$
\end{corollary}
\begin{proof}
  We take $A=U\Sigma V^*$ as its SVD where $U, V$ are both $n\times n$ unitary and let $S^+=V_r\Sigma_r^{-1/2}U_r^*$. By [7, Theorem 7.3.1], $P_1=(AA^*)^{1/2}=(U\Sigma V^*V\Sigma U^*)^{1/2}=U\Sigma U^*$, and $P_2=(A^*A)^{1/2}=(V\Sigma U^*U\Sigma V^*)^{1/2}=V\Sigma V^*$. Therefore, $P_1^{1/2}=U\Sigma^{1/2}U^*$ and $P_2=V\Sigma^{1/2}V^*$ which leads to $(P_1^{1/2})^+=U_r\Sigma_r^{-1/2} U_r^*$ and $(P_2^{1/2})^+=V_r\Sigma_r^{-1/2} V_r^*$. Recall the third and seventh line in (39), we have \begin{equation*}
\begin{aligned}
     k&=\|(P_1^{1/2})^+E(P_2^{1/2})^+\| \\
    &=\|U_r\Sigma_r^{-1/2}U_r^* E V_r\Sigma_r^{-1/2}V_r^* \|\\
    &\overset{(39)}{=}\|V_r\Sigma_r^{-1/2} U_r^* E V_r\Sigma_r^{-1/2}U_r^* \| \\ 
    &=\|S^+ES^+\|
    \end{aligned}
\end{equation*}
We can now apply Theorem 4.1 to $A, E$ with $m=n$ since $\|S^+ES^+\|=k\leq 1$ and replace $\|S^+ES^+\|$ with $k=\|(P_1^{1/2})^+E(P_2^{1/2})^+\|$ since they are equal, hence obtain (42) for $i\in \{1,...,2r-n\}$, and (43) for $i\in \{1,...,r\}$.
\end{proof}
In particular, when $A$ is $n\times n$ non-singular, all $\sigma_i(A)$ are positive. Setting $r=n$ and pseudo inverse to be normal inverse in Corollary 4.1.2, we get for $i\in \{1,...,n\}$,\begin{equation*}
\begin{array}{cc}
\sigma_{i}(A+E)-\sigma_i(A)\leq k\sigma_i(A), &\sigma_{i}(A+E)-\sigma_i(A)\geq -k\sigma_i(A)\\
\end{array}
    \end{equation*}
which means \begin{equation*}
    \frac{|\sigma_i(A+E)-\sigma_i(A)|}{\sigma_i(A)}\leq k
\end{equation*}
 where $k=\|P_1^{-1/2}EP_2^{-1/2}\|=\|S^+ES^+\|\leq 1$. Hence, we recover Theorem 3.1 in [4].

 When $A$ is normal, let $A=VDV^*$ be its spectral decomposition where its eigenvalues are ordered in decreasing modulus value. Then $A=V\mbox{sign}(D)|D|V^*$ is an SVD of $A$, so $\sigma_i(A)=|\lambda_i(A)|$ for $i\in \{1,...,n\}$. Let $k=\|(A^{1/2})^+E(A^{1/2})^+\|$ and $A+E$ be also normal. Using Corollary 4.1.2 and (4),  one could get $|\lambda_{2n-2r+i}(A+E)|\leq (1+k)|\lambda_i(A)|$ for $i\in \{1,..., 2r-n\}$, and 
$|\lambda_i(A+E)|\geq (1-k)|\lambda_i(A)|$ for $i\in \{1,..., r\}$ as Weyl-type relative bounds. However, $A+E$ is not normal in general even when both $A,E$ are normal, unless they are simultaneously diagonalisable, which is why it is hard to establish additive perturbation results for eigenvalues of normal matrices, besides the Bauer-Fike Theorem in [1].

\textbf{Acknowledgements.}  I would like to thank Professor Y. Nakatsukasa for being my supervisor of this dissertation who provided me with clear guidance and helpful advice.


==> contents.tex/Introduction.tex <==
\section{Introduction and preliminaries}
Given a square matrix $A$, it has been an active research area to give bounds on the eigenvalues of $A+E$ in terms of eigenvalues of $A$, where $E$ can be interpreted differently, such as a general additive perturbation to $A$, or a matrix arises due to floating-point errors as considered in [11]. When both $A$ and $E$ are Hermitian, the Weyl's bound gives \begin{equation*}
  -\|E\| \leq \lambda_i(A+E)-\lambda_i(A)\leq \|E\|
\end{equation*}
for $i\in \{1,...,n\}$, establishing a one-to-one pairing between $\lambda_i(A+E)$ and $\lambda_i(A)$ for the same index $i$, and in general a perturbation bound with such correspondence is classified as a Weyl-type bound in [6] and [8]. The Weyl's bound belongs to absolute perturbation results as it concerns the absolute difference between $\lambda_i(A+E)$ and $\lambda_i(A)$, whereas another important category of perturbation results is relative bounds that consider the relative difference between $\lambda_i(A+E)$ and $\lambda_i(A)$. There have been many relative bounds developed in research such as [4, 5, 6, 8, 10, 11] and in particular, the Weyl-type relative bounds always 
 take the form \begin{equation*}
    -k|\lambda_i(A)|\leq \lambda_i(A+E)-\lambda_i(A) \leq k|\lambda_i(A)|
\end{equation*}
for $i\in \{1,...,n\}$ where different constants $k$ correspond to different relative bounds. An assumption for these results which is always made is that $A$ is Hermitian non-singular
and $E$ is Hermitian, for example, $A$ and $A+E$ are taken to be positive definite in [6, 8, 10]. In contrast, the Weyl's bound above just requires both $A$ and $E$ to be Hermitian. Hence, in this dissertation our main goal is to extend the existing Weyl-type relative perturbation bounds to the case that $A$ may not have full rank, so to apply these relative bounds we do not need stronger assumptions on the structure of $A$ and $E$ than to apply the Weyl's bound. 

In section 2, we will first establish a relative bound in Theorem 2.1 which extends [4, Theorem 2.1] considering the case that $A$ have rank $r\leq n$. To follow, we will use this result to give a class of Weyl-type relative perturbation results that not only incorporate all the major Weyl-type relative bounds in [4, 5, 6, 8, 10] but also take into account that $A$ is potentially singular, achieving our principal objective. 

It will be revealed that the sharpness of the bound in Theorem 2.1 depends on the $i$th eigenvalue of $A$ whereas the Weyl's bound is invariant with respect to the indices, so we will investigate for which indices the relative bound is likely to be sharper than the Weyl's bound in Section 3. Also, we will look into a known relation between Theorem 2.1 and congruence transformation but additionally consider the case that $A$ could be singular.

Using Theorem 2.1, the existing relative perturbation bounds for singular values can be also extended to a more general case via the Jordan-Wielandt matrices, which we will discuss in Section 4.  

We will next quickly introduce some notations and results that we will be using.

 We let $A^*$ denote the Hermitian of $A$. When both $A$ and $B$ are Hermitian, we denote $A\geq \mathbf{0}$ if $A$ is positive semi-definite, and $B\leq A$ if $A-B$ is positive semi-definite.  When $A$ is normal, it has a unitarily diagonalisation as $A=VDV^*$ where $D=\mbox{diag}(\lambda_1, ..., \lambda_n)$ with entries being the eigenvalues of $A$ and $V$ is unitary. We can always arrange its eigenvalues to be decreasing with respect to the indices which is our default ordering when $A$ is non-singular. When $A$ may not have full rank, the specified ordering we will use is $\lambda_1\geq...\geq \lambda_r, \lambda_{r+1}=...=\lambda_n=0$ where $r=\mbox{rank}(A)$. 

When $A$ is normal, we define $A^{1/2}$ to be any normal matrix so that $(A^{1/2})^2=A$ as in [4]. It has  an equivalent characterisation in terms of its diagonal eigenvalue matrix:  since $AA^{1/2}=(A^{1/2})^2A^{1/2}=A^{1/2}(A^{1/2})^2=AA^{1/2}$ and both $A^{1/2}, A$ are normal, if $A=VDV^*$ as its unitary diagonalisation then $A^{1/2}=V\Lambda V^*$ where $\Lambda$ is diagonal, using [7, Theorem 2.5.5]. Since $(A^{1/2})^2=V\Lambda^2 V^*=VDV^*=A$, $\Lambda^2=D$ so $\Lambda =D^{1/2}$, which means $A^{1/2}=VD^{1/2}V^*$. On the other hand, if $A^{1/2}=VD^{1/2}V^*$ then it is normal and $(A^{1/2})^2=VDV^*=A$. There can be different choices of $D^{1/2}$ but their 2-norm are the same, since any two of them differ by a diagonal matrix with entries being roots of unity. Hence all choices of $A^{1/2}$ have the same 2-norm, so it is well-defined to consider the 2-norm of $A^{1/2}B$, $CA^{1/2}$ or $A^{1/2}EA^{1/2}$ for any matrices $B, C, E$ by the unitary invariance of 2-norm. If $\mbox{rank}(A)=r$ and $A=VDV^*=V_rD_rV_r^*$ as its thin unitary diagonalisation, since $0^{1/2}=0$, $A^{1/2}=VD^{1/2}V^*=V_rD_r^{1/2}V_r^*$.

Any matrix $A$ has a SVD $A=U\Sigma V^*$ where $\Sigma=\mbox{diag}(\sigma_1, ..., \sigma_n)$ with entries being the singular values of $A$ which are non-negative and decreasing with respect to the indices, and $V$ is unitary, $U$ is orthonormal which is unitary when $A$ is a square matrix. Starting from its SVD, every square matrix $A=U\Sigma V^*$ has a left and right polar decomposition $A=P_1S=SP_2$ where $P_1=U\Sigma U^*=(AA^*)^{1/2}$ and $P_2=V\Sigma V^*=(A^*A)^{1/2}$ are positive semi-definite, and $S=UV^*$ is unitary. When $A$ is normal, its left and right polar factor coincide and $A=PS=SP$, as the polar factor is uniquely determined to be $P=(A^*A)^{1/2}=(AA^*)^{1/2}$ by [7, Theorem 7.3.1]. If $A=VDV^*$ as its unitary diagonalisation, $P=(A^*A)^{1/2}=V|D|V^*$.

We let $\|A\|$ denote the 2-norm of $A$, which is $\sigma_1$ its largest singular value. For any square matrix $A$, we have $\|A\|\geq \max\limits_i|\lambda_i(A)|$, because if we take its Schur's decomposition [7, Theorem 2.3.1], $\|A\|=\|QTQ^*\|=\|T\|\geq \max\limits_i|\lambda_i(A)|$. In particular, when $A$ is Hermitian, $\|A\|=\|VDV^*\|=\|D\|=\max\limits_i|\lambda_i(A)|=|\lambda_{j^*}(A)|$ for some index $j^*$.

For any matrix $A$, we let $A^+$ denote its unique pseudo inverse, which is defined to  satisfy 1) $AA^+A=A$, 2) $A^+AA^+=A^+$, 3) $A^+A$ is Hermitian, 4) $AA^+$ is Hermitian.  An equivalent definition for $A^+$ which we will use is if $A=U\Sigma V^*=U_r\Sigma_rV_r^*$ is its thin SVD where $r=\mbox{rank}(A)$, then $A^+=V_r\Sigma_r^{-1}U_r^*$. When $Q, W$ are unitary, $(QAW)^+=W^*A^+Q^*$ using the second definition.





==> contents.tex/References.tex <==

\section*{References}
[1] F.L. Bauer, C.T. Fike, \textit{Norms and exclusion theorems}, Numer. Math. 2 (1960) 137-141. \\\relax
[2] R. Bouldin, \textit{The pseudo-inverse of a product}, SIAM J. Appl. Math. 24 (1973) 489-495. \\\relax
[3] J. Demmel, K. Veselić, \textit{Jacobi’s method is more accurate than QR}, SIAM J. Matrix Anal. Appl. 13
(1992) 1204–1245. \\\relax
[4] F.M. Dopico, J. Moro, J.M. Morela, \textit{Weyl-type relative perturbation bounds for eigensystems of Hermitian matrices}, Linear Algebra Appl. 309 (2000) 3-18.\\\relax
[5] S.C. Eisenstat, I.C.F. Ipsen, \textit{Relative perturbation techniques for singular value problems}, SIAM
J. Numer. Anal. 32 (1995) 1972-1988.\\\relax 
[6] S.C. Eisenstat, I.C.F. Ipsen, \textit{Three absolute perturbation bounds for matrix eigenvalues imply relative bounds}, SIAM J. Matrix Anal. Appl. 20 (1998) 149-158. \\\relax
[7] R.A. Horn, C.R. Johnson, \textit{Matrix Analysis}, second ed., Cambridge University Press, Cambridge, 2013. \\\relax
[8] I.C.F. Ipsen, \textit{Relative perturbation results for matrix eigenvalues and singular values}, Acta Numer. 7 (1998) 151-201.\\\relax
[9] S. Izumino,  \textit{The product of operators with closed range and an extension of the reverse order law}, Tôhoku Math. J. 34 (1982) 43-52.\\\relax
[10] R. Mathias, \textit{Spectral perturbation bounds for positive definite matrices}, SIAM J. Matrix Anal. Appl. 18 (1997) 959-980.\\\relax
[11] K. Veselić, I. Slapničar, \textit{Floating-point perturbations of Hermitian matrices}, Linear
Algebra Appl. 195 (1993) 81-116. \\\relax

